ClearBuds: Wireless Binaural Earbuds for Learning-Based Speech Enhancement

We present ClearBuds, the first hardware and software system that utilizes a neural network to enhance speech streamed from two wireless earbuds. Real-time speech enhancement for wireless earbuds requires high-quality sound separation and background cancellation, operating in real-time and on a mobile phone. Clear-Buds bridges state-of-the-art deep learning for blind audio source separation and in-ear mobile systems by making two key technical contributions: 1) a new wireless earbud design capable of operating as a synchronized, binaural microphone array, and 2) a lightweight dual-channel speech enhancement neural network that runs on a mobile device. Our neural network has a novel cascaded architecture that combines a time-domain conventional neural network with a spectrogram-based frequency masking neural network to reduce the artifacts in the audio output. Results show that our wireless earbuds achieve a synchronization error less than 64 microseconds and our network has a runtime of 21.4 milliseconds on an accompanying mobile phone. In-the-wild evaluation with eight users in previously unseen indoor and outdoor multipath scenarios demonstrates that our neural network generalizes to learn both spatial and acoustic cues to perform noise suppression and background speech removal. In a user-study with 37 participants who spent over 15.4 hours rating 1041 audio samples collected in-the-wild, our system achieves improved mean opinion score and background noise suppression. Project page with demos: https://clearbuds.cs.washington.edu

==> abstract-1.tex <==

\begin{abstract}
With the rapid proliferation of headsets and wireless earbuds, more people than ever are taking calls in noisy environments on-the-go.
%--- on the street, in open office environments, or at the grocery store --- 
%Speech enhancement seeks to clean noisy speech input to provide a more pleasant experience for the person at the other end of the line.
To realize a practical speech enhancement system for consumers, multiple criteria must be met. The system must effectively remove background noise, including undesired speech sources, operate in real-time, and be deployed at par with the wireless earbud form factors consumers have come to expect.
Traditional microphone beamforming techniques in headsets provide limited attenuation of background noise and voices. While single-channel speech enhancement networks can better suppress noise, they are unable to distinguish and attenuate undesired background voices due to their lack of spatial filtering.
%Traditional microphone beamforming techniques in headsets and learned, single-channel speech enhancement networks are each challenged by non-stationary noise sources and undesired background speech, respectively. 
%We recognize the unique placement of microphones in earbuds, can offer
We present Clearbuds, a system consisting of a set of synchronized, wireless earbuds and a lightweight, dual-channel speech enhancement network deployed on a mobile phone.
The network learns both spatial cues that beamform toward the user's mouth and acoustic cues that filter on voice priors.
Experiments at the network-level and system-level show that ClearVoice exceeds larger single-channel networks and beamformed systems in terms of suppressing background noise (by XX dB SDR), background speech (by XX dB SDR), and mixtures (by XX dB SDR), all while operating within the computational constraints of a mobile device at XX ms latency.


\end{abstract}

==> accessibility_figure_descriptions.tex <==
Figure 1. The left image are white earbuds, round in shape. The right image is the PCB out of the plastic covering sitting next to a quarter. They are approximately the same size.

Figure 2. A block diagram of the system set up. A cartoon of the users head (top view) sits in the center with a microphone in each ear. Blocks indicating noise  and background voice are placed to each side emitting red signals to be blocked. The mouth is emitting green signals to be enhanced. The microphone blocks each have an arrow to a phone block. The phone block sends three arrow (noise, voice, and background voice) to the ClearBuds network. Only one green arrow labeled voice emerges from ClearBuds Network block and goes to a block called telephony.

Figure 3. Network diagram. On the left are two waveforms labeled L channel and R channel inputs. Arrow emerge splitting down two paths. The top path has both L and R going into a CB-Conv-TasNet block, then to an output waveforms, then to an FFT, where a spectrogram image is depicted. The bottom path adds the two L and R waveforms which then go to an input spectrogram image then to a CB-UNet block then to a CB-Unit Output block with a spectrogram mask image. The top and bottom mask are combined via multiply to yield a CB-Net Spectrogram image. This is fed into an IFFT block and then an output is depicted.

Figure 4. Contains four heat map images of spectrograms. The first is the mixture. It has the most variation in intensity. The next is CB-Conv-TasNet. There is an inset pointing to a particular section. The next is CB-Net, there is also an inset. The last is GT, there is also an inset. In the inset, the CB-Net looks more similar to GT than to CB-Conv-TasNet image indicating successful clean up of noise.

Figure 5. A neural network diagram of the ClearBuds Conv-TasNet. At the bottom is 1.59 seconds of audio input. Arrows connect this input to many circles arranged horizontally, depicting the first neural network layer. There are several layers of network connections with arrows pointing upward with progressively fewer neurons in each layer. At the very top is a single box labeled "output 350 samples". An arrow connects a small part of the input audio file to the output sample, illustrating a skip connection.

Figure 6. The figure has two separate images. On the left is a schematic of the ClearBud circuit board. The largest component is labeled BLE corresponding to the Bluetooth component. Additional components include a coin cell, micro USB B, external microphone, accel, flash, and two LEDS. On the right is a photo depicting the ClearBuds earbuds, next to a quarter for size. Each ear piece is circular and roughly the size of a quarter. One earbud does not have a case and the circuit board is visible. The others contain a rubber tip and a plastic case for holding in the ear.

Figure 7. This figure is a block diagram showing how the time sync process works between two wireless earbuds. On the left hand side there are blocks showing how microphone data gets clocked into PCM buffers inside RAM. To maintain time sync, the secondary ClearBud has custom blocks which receive a Primary Sync Clock which is connected to the Rate Encoder, controlling the secondary PCM Buffer size. The PCM buffer then points to a 2 factor decimator, which then gets outputted to a ring buffer. The ring buffer then has an arrow indicating it outputs into a BLE Data Packer. This then has another arrow expanding upon what each BLE Packet looks like at the byte level. Finally, there is an arrow from here connecting it to the BLE hardware operating at 2Mbps.

Figure 8. A line graph with minutes elapsed on x-axis. Goes from 0 to 5 minutes. Time error (us) on the y-axis from 0 to 640us). A red line representing time sync off rises linearly from (0,0) to (5, 640). A blue line indicating time sync on fluctuates between 0 and 64 us but never exceed 64 us.

Figure 9.  Bar graph indicating noise suppression and mean opinion score. Values are all captured in paper text. 95\% CI are indicated. They are about a similar size for all bars (about plus or minus 0.2).

Figure 10. There are three line graphs. The first is Angle of Background Voice on the x-axis and SI-SDRi on the y axis. Around 0 degrees, the SI-SDRi is around 3, and the line increase sharply until 20 degrees when the SI-SDRIi is around 10. It then increase gradually to 90 degrees where the SI-SDRIi is around 12. The second graph is Reverb vs SI-SDRi. Around 0 reverb the SI-SDRi is 10, and the line decreases gradually to a reverb value of 4.0 and SI-SDRIi of 8. The last graph is Ear Distance vs SI-SDRi. The graph is roughly flat around 10 SI-SDRI for Ear Distances of 10cm to 25cm. 


==> sections/1-OLDintro-2.tex <==
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With the rapid proliferation of wireless earbuds, more people than ever are taking calls on-the-go. Apple alone sold more than 100 million AirPods in 2020.  While these systems offer unprecedented convenience, their mobility raises an important technical challenge: on a call, environmental sounds, such as street noises, machinery, and other people talking, interfere with the target speech and affect voice quality. %, hindering the ability to clearly communicate. 

%Apple AirPods alone have approximately doubled in sales each year since 2017, surpassing 100 million units sold in 2020~[{xx}].

\begin{ready-for-review}


Existing wireless earbuds are limited in their ability to provide speech enhancement under such noisy conditions. They typically use beamforming which requires low latency computation on local digital signal processors. Further, they communicate via Bluetooth which supports only a single-channel uplink in hands-free profile mode. The combination of the two results in beamforming  performed using two microphones on a single earbud in an end-fire configuration~[xxx]. This makes the conveniently small size of these devices a double-edged sword: the small separation between microphones on a single earbud reduces beamforming gains. Furthermore, signal processing-based beamforming techniques do not incorporate acoustic cues found in a human voice, limiting their ability to effectively perform speech enhancement~[xxx,xxx].  Deep learning methods have demonstrated promising speech enhancement performance using a single microphone [xxx,xxxx,xxx]. However, such systems do not perform well in situations where multiple human speakers are present, since a single microphone model lacks the spatial information required to isolate the intended speaker. %Recently, multi-channel source separation algorithms have shown impressive results isolating a target source via wired microphone arrays.

We present the first system that uses neural networks to achieve real-time speech enhancement using wireless earbuds. Our key insight is to treat binaural wireless earbuds as a microphone array that can filter the wearer's voice on both spatial information and acoustic speech cues. Since the separation between the two wireless earbud is larger than two microphones on a single earbud, this approach can provide better spatial resolution.

To achieve this system, we make two key contributions spanning wireless hardware and deep learning. 

First, we designed a set of  wireless earbuds shown in Fig.~\ref{dsd} that maintain time synchronization between the microphones at a resolution of 32 microseconds and stream to a mobile device.  To our knowledge, this is one of the first systems to be able to synchronously stream each microphone channel from each earbud to the mobile phone. We expect our wireless earbud hardware (open-sourced at publication) to be of wider interest as a research and development platform.

Second, we introduce a neural network that utilizes binaural input from wearable headphones to isolate the target speaker based on both voice and spatial information. We designed our network to run real-time on a mobile device with latencies of XX-XX~ms across a variety of devices. To achieve real-time operation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 22.4ms, we could re-use 98\% of the computed network activations from the previous time step for each new audio segment. Experiments show that our network outperforms a number of baselines on both synthetic and real data.


We combine our wireless earbuds and network to create ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time, on-device processing on a commodity mobile phone paired to set of wireless earbuds. 

\end{ready-for-review}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Imagine a world a in 

% They cannot do two channel because of bluetooth reasons

% They are doing beamforming on one device

% What is the first thing that we're doing

% What's novel about the end to end system, it's real time, on the mobile device, using two mics

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Background noise during phone and video calls is a persistent problem that affects people all over the world. Environmental sounds, such as street noises, machinery noises, or other people talking, can be transmitted along with the speaker, which hinders the ability to clearly communicate.

% Speech enhancement is the task of isolating the speaker of interest and suppressing all unwanted background sounds. Recently, there have been many advances in machine learning that attempt to remove these artifacts from a single microphone input. Such systems do not perform well in situations where multiple human speakers are present due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker. In addition, such systems generally perform worse than those that utilize multiple microphones.  

%  We are particularly motivated by the rise in multi-microphone wearable headphones in everyday settings. Examples include AirPods and PixelBuds, which have become increasingly popular in recent years. Although these devices often employ some amount of directional pickup, via beamforming or microphone design, these mechanisms offer limited attenuation of background noise compared to deep learning methods.
 
%  In contrast to these approaches, we propose a neural network that utilizes binaural input from wearable headphones in order to isolate the target speaker based on both voice and spatial information. Furthermore, we design our network to run real-time on a mobile device and show low latency across a variety of devices. To achieve real-time separation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 50ms, we can re-use 99\% of the computed network activations from the previous time step for each new segment of audio. Experiments show that our network can outperform a number of baselines on both synthetic and real data.
 
%  As a further contribution, we designed a set of wireless earbuds that maintain time synchronization between the microphones at a resolution of 32 microseconds. We built a custom wireless protocol over Bluetooth Low Energy (BLE) to enable synchronized, two-channel microphone streaming to the mobile device. To our knowledge, this is one of the first systems to be able to synchronously stream each microphone channel from each earbud to the mobile phone. This represents a step forward from single earbud beam-forming techniques, which were designed around the fact that current Bluetooth audio protocols only support one microphone channel for uplink. We expect our wireless earbuds to be of wider interest to the spatial audio community as a research and development platform.
 
% %  Because the current Bluetooth hands-free profile (HFP) only supports one microphone for uplink, 
 
% %  This represents a step forward from traditional single-side, on-device beam-forming techniques, and we expect our technique to be of wider interest to the spatial audio community.
 
%  We combine the neural network with our headphones to create a system called ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%

% For most use cases, speech enhancement systems must run in real-time on the hardware available. This hardware includes both the microphone available as well as the processing hardware. Although many previous works use a single microphone along with a GPU or a laptop CPU,


% In contrast to traditional speech enhancement techniques, we notice that the geometry of the mouth with respect to earbuds allows us to apply an additional geometric heuristic, which then allows us to adapt source separation techniques to speech enhancement. xxxxxx

% In contrast to more general purpose source separation formulations, the key insight is that for speech enhancement on wireless earbuds, the goal is to focus on the voice source  that is approximately equidistant from the two earbuds. 

% To separate the wearer's voice we train a neural network to separate voice sources that are in the center of the microphone array. We use a similar technique as Cone-of-Silence, but do not need the location conditioning variables because the target speaker is always in a known position. xr

% P1
% (1) Succinctly define the problem. Need speech enhancement on earbuds. Focusing on the person who is talking.
% (2) This is useful because people are talking while walking around (buses, streets) with wireless earbuds, existing approaches are not equipped to solve this.

% P2
% Beamforming, why they don't work. 2-3 academic citations, limited because of this reason. 
% On the other hand neural networks have done single channel, but they are limited due to .
% Synthetic data , non causal

% P3
% We built xxx. Key insight to make this realtime is xx. Built system which can wirelessly stream this thing and collected real data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textcolor{red}{Shyam: This history lesson is not required.}
%  In all aspects of our daily lives, the ability for us to hold conversations from one to another anywhere around the world has become an ability that is important in both our personal and work lives. Engineering efforts continue to push the telephony experience by improving voice quality, reducing latency, and eliminating background noise for a better experience. Finally, the advent of telephony has also contributed toward the rapid advancement of audio devices such as wireless earbuds and headsets for both improved voice quality and the ability to take calls hands-free.

% % Improvements in the telephony experience also extend into the video domain. Video calls and video conferencing have been established so that we can now see each other’s faces to further improve the experience of effectiveness of our ability to communicate and collaborate with each other. In the work environment especially, video conferencing has become a necessity for employees and collaborators working from home and working remotely. Indeed, the SARS-CoV-2 (COVID-19) pandemic has only exacerbated this need, as the need for effective video conferencing software (Zoom, Microsoft Teams, Cisco Webex) has become a staple for us to remain effective while we work from home.

% \textcolor{red}{In efforts to continue to improve the telephony experience, engineering innovations are made across both the hardware and software space. For example, digital MEMS microphones have long been preferred to their analog counterparts for noise immunity in wireless audio systems with high frequency radio components.} Today’s phones and wireless earbuds have also taken a step further by adding beam-forming to amplify a speaker’s voice while attenuating external background noise. While the strengths of beam-forming become stronger with distance between two microphones, companies like Apple and Google still integrate dual microphones on their wireless earbuds like AirPods and PixelBuds to gain the benefits of beam-forming microphones. While beam-forming functions well on these edge devices, its ability to attenuate non-broadband-noise fall short. Noises such as loud buses and subways, home appliances, and other background voices persist in the audio uplink during a voice call, disrupting the overall communication experience.

% Recently, developments in the machine learning space have attempted to remove these extremities from a single microphone channel. These networks operate by utilizing spectrogram transformations to learn human voice priors, thus retaining human speech while eliminating other noises. While research continues in the academic space, companies like Krisp have begun to productize this technology so that people can enjoy voice and video calls with background noise removal in the uplink channel. Interest in this technology has also influenced companies like Google, as they recently introduced background noise cancellation on their video conferencing platform, Google Meet.

% While Krisp and Google Meet perform well to isolate human speakers while eliminating background noise, they do not perform well in situations where multiple human speakers are present. This is primarily due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker in respect to surrounding background voices. This is a nontrivial pitfall, as the ability for these networks to remove noise and background voices in environments such as cafes, call centers, or shared work spaces become weaker.

% To combat this, we introduce and propose ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. The basis of our contributions function by integrating both the advances in the wireless earbud ecosystem along with audio source separation networks in the deep learning space. Specifically, we architect and engineer a solution which streams microphone data from both a user’s left and right ear as inputs for our source separation network. With two input channels, our network now attains the spatial information required to eliminate background voices while also isolating the intended speaker, which should be spatially equidistant between a pair of wireless earbuds.

% The contributions of this approach are feasible with our end-to-end system which consists of a pair of wireless earbuds and a mobile phone. Custom firmware is embedded in each earbud which maintains time synchronization between the microphones at a resolution of 32 microseconds. Additionally, a custom wireless protocol is designed to stream the time-synced microphones in real-time to a mobile phone for processing. To our knowledge, this is the first system in which multiple wireless microphones are leveraged to expand upon commercially available background noise cancellation voice technologies (Krisp, Google Meet). Transitively, this is also the first demonstration of streaming both microphones in a pair of wireless earbuds, taking a step forward from traditional single-side, on-device beam-forming techniques. We present comparative results to show that we perform comparatively against non-causal [deep learning model] by xxx dB, while outperforming commercially available models (Krisp) by xxx dB and on-device beam-forming (AirPods) by xxx dB. 

==> sections/1-intro-3.tex <==
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With the rapid proliferation of wireless earbuds (100 million AirPods sold in 2020), more people than ever are taking calls on-the-go.  While these systems offer unprecedented convenience, their mobility raises an important technical challenge:  environmental noise (street sounds, people talking, etc.) can interfere and make it harder to understand the speaker.
We therefore seek to enhance the speaker's voice, and suppress background noise.

We present the first system that uses neural networks to achieve real-time speech enhancement from binaural wireless earbuds. 
Our key insight is to treat wireless earbuds as a binaural microphone array,
and exploit the specific geometry -- two well-separated microphones behind a proximal source -- to devise a specialized neural network for high quality speaker separation.

Achieving this goal is challenging, as today's earbuds aren't capable of operating in this manner; AirPods and similar devices upload microphone output from only a single earbud at a time, a limitation of the Bluetooth standard\footnote{Beam forming is limited to multiple mics {\em on the same earbud}.}.  To achieve binaural speaker separation, we 
therefore designed and built novel prototype earbud hardware on which to deploy our deep learning speaker separation approach.

To achieve this system, we make two key contributions spanning wireless hardware and deep learning. 
First, we designed a pair of wireless earbuds, shown in Fig.~\ref{fig:earbuds},
capable of streaming two time-synchronized microphone audio streams to a mobile device.  This is one of the first systems of its kind, and we expect our wireless earbud hardware (open-sourced at publication) to be of wider interest as a research and development platform.  
We did the design in an academic lab (DIY) using open source eCAD software, outsourced fabrication and assembly to PCBWay in China ($\$2$K for 50 units), and 3D printed our own enclosures.

Second, we introduce a neural network that utilizes binaural input from wearable earbuds to isolate the target speaker.
%based on both voice and spatial information. 
We designed our network to run in real-time on a mobile device with latencies of 17.5--27.2~ms across a variety of devices. To achieve real-time operation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 50ms, we achieved re-use of 99\% of the computed network activations from the previous time step for each new audio segment. Experiments show that our network outperforms a number of baselines on both synthetic and real data.


We combine our wireless earbuds and network to create ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time, on-device processing on a commodity mobile phone paired to set of wireless earbuds. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Imagine a world a in 

% They cannot do two channel because of bluetooth reasons

% They are doing beamforming on one device

% What is the first thing that we're doing

% What's novel about the end to end system, it's real time, on the mobile device, using two mics

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Background noise during phone and video calls is a persistent problem that affects people all over the world. Environmental sounds, such as street noises, machinery noises, or other people talking, can be transmitted along with the speaker, which hinders the ability to clearly communicate.

% Speech enhancement is the task of isolating the speaker of interest and suppressing all unwanted background sounds. Recently, there have been many advances in machine learning that attempt to remove these artifacts from a single microphone input. Such systems do not perform well in situations where multiple human speakers are present due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker. In addition, such systems generally perform worse than those that utilize multiple microphones.  

%  We are particularly motivated by the rise in multi-microphone wearable headphones in everyday settings. Examples include AirPods and PixelBuds, which have become increasingly popular in recent years. Although these devices often employ some amount of directional pickup, via beamforming or microphone design, these mechanisms offer limited attenuation of background noise compared to deep learning methods.
 
%  In contrast to these approaches, we propose a neural network that utilizes binaural input from wearable headphones in order to isolate the target speaker based on both voice and spatial information. Furthermore, we design our network to run real-time on a mobile device and show low latency across a variety of devices. To achieve real-time separation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 50ms, we can re-use 99\% of the computed network activations from the previous time step for each new segment of audio. Experiments show that our network can outperform a number of baselines on both synthetic and real data.
 
%  As a further contribution, we designed a set of wireless earbuds that maintain time synchronization between the microphones at a resolution of 32 microseconds. We built a custom wireless protocol over Bluetooth Low Energy (BLE) to enable synchronized, two-channel microphone streaming to the mobile device. To our knowledge, this is one of the first systems to be able to synchronously stream each microphone channel from each earbud to the mobile phone. This represents a step forward from single earbud beam-forming techniques, which were designed around the fact that current Bluetooth audio protocols only support one microphone channel for uplink. We expect our wireless earbuds to be of wider interest to the spatial audio community as a research and development platform.
 
% %  Because the current Bluetooth hands-free profile (HFP) only supports one microphone for uplink, 
 
% %  This represents a step forward from traditional single-side, on-device beam-forming techniques, and we expect our technique to be of wider interest to the spatial audio community.
 
%  We combine the neural network with our headphones to create a system called ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%

% For most use cases, speech enhancement systems must run in real-time on the hardware available. This hardware includes both the microphone available as well as the processing hardware. Although many previous works use a single microphone along with a GPU or a laptop CPU,


% In contrast to traditional speech enhancement techniques, we notice that the geometry of the mouth with respect to earbuds allows us to apply an additional geometric heuristic, which then allows us to adapt source separation techniques to speech enhancement. xxxxxx

% In contrast to more general purpose source separation formulations, the key insight is that for speech enhancement on wireless earbuds, the goal is to focus on the voice source  that is approximately equidistant from the two earbuds. 

% To separate the wearer's voice we train a neural network to separate voice sources that are in the center of the microphone array. We use a similar technique as Cone-of-Silence, but do not need the location conditioning variables because the target speaker is always in a known position. xr

% P1
% (1) Succinctly define the problem. Need speech enhancement on earbuds. Focusing on the person who is talking.
% (2) This is useful because people are talking while walking around (buses, streets) with wireless earbuds, existing approaches are not equipped to solve this.

% P2
% Beamforming, why they don't work. 2-3 academic citations, limited because of this reason. 
% On the other hand neural networks have done single channel, but they are limited due to .
% Synthetic data , non causal

% P3
% We built xxx. Key insight to make this realtime is xx. Built system which can wirelessly stream this thing and collected real data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textcolor{red}{Shyam: This history lesson is not required.}
%  In all aspects of our daily lives, the ability for us to hold conversations from one to another anywhere around the world has become an ability that is important in both our personal and work lives. Engineering efforts continue to push the telephony experience by improving voice quality, reducing latency, and eliminating background noise for a better experience. Finally, the advent of telephony has also contributed toward the rapid advancement of audio devices such as wireless earbuds and headsets for both improved voice quality and the ability to take calls hands-free.

% % Improvements in the telephony experience also extend into the video domain. Video calls and video conferencing have been established so that we can now see each other’s faces to further improve the experience of effectiveness of our ability to communicate and collaborate with each other. In the work environment especially, video conferencing has become a necessity for employees and collaborators working from home and working remotely. Indeed, the SARS-CoV-2 (COVID-19) pandemic has only exacerbated this need, as the need for effective video conferencing software (Zoom, Microsoft Teams, Cisco Webex) has become a staple for us to remain effective while we work from home.

% \textcolor{red}{In efforts to continue to improve the telephony experience, engineering innovations are made across both the hardware and software space. For example, digital MEMS microphones have long been preferred to their analog counterparts for noise immunity in wireless audio systems with high frequency radio components.} Today’s phones and wireless earbuds have also taken a step further by adding beam-forming to amplify a speaker’s voice while attenuating external background noise. While the strengths of beam-forming become stronger with distance between two microphones, companies like Apple and Google still integrate dual microphones on their wireless earbuds like AirPods and PixelBuds to gain the benefits of beam-forming microphones. While beam-forming functions well on these edge devices, its ability to attenuate non-broadband-noise fall short. Noises such as loud buses and subways, home appliances, and other background voices persist in the audio uplink during a voice call, disrupting the overall communication experience.

% Recently, developments in the machine learning space have attempted to remove these extremities from a single microphone channel. These networks operate by utilizing spectrogram transformations to learn human voice priors, thus retaining human speech while eliminating other noises. While research continues in the academic space, companies like Krisp have begun to productize this technology so that people can enjoy voice and video calls with background noise removal in the uplink channel. Interest in this technology has also influenced companies like Google, as they recently introduced background noise cancellation on their video conferencing platform, Google Meet.

% While Krisp and Google Meet perform well to isolate human speakers while eliminating background noise, they do not perform well in situations where multiple human speakers are present. This is primarily due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker in respect to surrounding background voices. This is a nontrivial pitfall, as the ability for these networks to remove noise and background voices in environments such as cafes, call centers, or shared work spaces become weaker.

% To combat this, we introduce and propose ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. The basis of our contributions function by integrating both the advances in the wireless earbud ecosystem along with audio source separation networks in the deep learning space. Specifically, we architect and engineer a solution which streams microphone data from both a user’s left and right ear as inputs for our source separation network. With two input channels, our network now attains the spatial information required to eliminate background voices while also isolating the intended speaker, which should be spatially equidistant between a pair of wireless earbuds.

% The contributions of this approach are feasible with our end-to-end system which consists of a pair of wireless earbuds and a mobile phone. Custom firmware is embedded in each earbud which maintains time synchronization between the microphones at a resolution of 32 microseconds. Additionally, a custom wireless protocol is designed to stream the time-synced microphones in real-time to a mobile phone for processing. To our knowledge, this is the first system in which multiple wireless microphones are leveraged to expand upon commercially available background noise cancellation voice technologies (Krisp, Google Meet). Transitively, this is also the first demonstration of streaming both microphones in a pair of wireless earbuds, taking a step forward from traditional single-side, on-device beam-forming techniques. We present comparative results to show that we perform comparatively against non-causal [deep learning model] by xxx dB, while outperforming commercially available models (Krisp) by xxx dB and on-device beam-forming (AirPods) by xxx dB. 

==> sections/1-intro-4.tex <==
\section{Introduction}




% From a user experience perspective, this would allow a user to not toggle the mute button on call, even when they are not speaking.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 4 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With the rapid proliferation of wireless earbuds (100 million AirPods sold in 2020~\cite{airpodssales}), more people than ever are taking calls on-the-go.  While these systems offer unprecedented convenience, their mobility raises an important technical challenge:  environmental noise (e.g., street sounds, people talking)  can interfere and make it harder to understand the speaker.
We therefore seek to enhance the speaker's voice, and suppress background sounds using speech captured across the two earbuds. 


Source separation of acoustic signals  is a long-standing problem where the conventional approach for decades has been to perform beamforming using multiple microphones. Signal processing-based beamformers that are computationally light-weight can encode the spatial information  but do not effectively capture the acoustic cues~\cite{van1988beamforming,krim1996two,chhetri2018multichannel}.  Recent work has shown that deep neural networks can encode both spatial and acoustic information and hence can  achieve superior source separation  with gains of up to $9$~dB over signal processing baselines~\cite{subakan2021attention,luo2019conv}. However, these neural networks are computationally expensive. None of the existing binaural (i.e., using two microphones) neural networks can  meet the end-to-end latency required for telephony applications or have been evaluated with real earbud data. Commercial end-to-end systems, like  Krisp~\cite{krisp}, use neural networks on a cloud server for single-channel  speech enhancement, with implications to  cost and privacy. % or on edge devices.


\begin{figure}[t!]
\centering
 \includegraphics[width=1\linewidth]{figures/flow-diagram-6.png}
\vskip -0.1in
\caption{\footnotesize{ ClearBuds Application.  Our goal is to isolate a user's voice from background noise (e.g., street sounds or other people talking) by performing source separation  using a pair of custom designed, synchronized, wireless earbuds.}}
\label{fig:block_diagram}
\vskip -0.15in
\end{figure}


%\footnote{The task of enhancing the wearer's  voice is for  telephony and video conferencing applications. This is not to be confused with active noise cancellation (ANC) which cancels out  noise coming to one's ears from an external environment~\cite{mute}.}

We present the first system that uses neural networks to achieve real-time speech enhancement from binaural wireless earbuds.
Our key insight is to treat wireless earbuds as a binaural microphone array,
and exploit the specific geometry -- two well-separated microphones behind a proximal source -- to devise a specialized neural network for high quality speaker separation. In contrast to using multiple microphones on the same earbud to perform beamforming, as is common in Apple AirPods \cite{airpods} and other hearing aids, we use microphones across the left and right earbuds, increasing the distance between the two microphones and thus the spatial resolution. 

Achieving this goal is challenging for three key reasons. First, today's earbuds are not capable of operating in this manner; AirPods and similar devices upload microphone output from only a single earbud at a time.  To achieve binaural speaker separation, we 
 need to design and build novel earbud hardware that can synchronously transmit audio data from both the earbuds. Second, binaural speech enhancement networks are not lightweight and have not been demonstrated with wireless earbuds. Reducing the network size naively often leads to unpleasant artifacts. Thus, we also need to optimize the neural networks to run in real-time on smart devices that have a limited computational capability compared to cloud GPUs. Further, we need to  meet the end-to-end latency requirements for telephony applications and ensure that the resulting audio output has a high quality from a user experience perspective. {Third, prior binaural  speech enhancement networks are trained and tested  on synthetic data and have not been shown to generalize well to real  data. Building an end-to-end system however requires a network that generalizes to in-the-wild real use.} 

\textcolor{red}{To achieve this system, we make two technical contributions spanning earable hardware and neural networks. 


\begin{figure}[t!]
\vskip -0.1in
\centering
\includegraphics[width=1\linewidth]{figures/clearbuds.png}
\vskip -0.15in
\caption{\footnotesize{ClearBuds hardware. The images show ClearBuds  inside 3D-printed enclosure and when  placed beside a quarter. }}
\label{fig:earbuds}
\vskip -0.15in
\end{figure}

\squishlist
\item {\bf Synchronized  binaural earables.} We designed a binaural wireless earbud system  (Fig.~\ref{fig:earbuds}) 
capable of streaming two time-synchronized microphone audio streams to a mobile device. This is one of the first systems of its kind, and we expect our earbud hardware and firmware (open-sourced at publication) to be of wider interest as a research and development platform. Existing earable platforms such as eSense~\cite{esense-1}  do not support time-synchronized audio transmission from two earbuds to a mobile device. 
We designed our DIY hardware  using open source eCAD software, outsourced fabrication and assembly to PCBWay ($\$2$K for 50 units), and 3D printed the  enclosures.

\item {\bf Light-weight cascaded neural network.} We introduce a light-weight  neural network  that utilizes binaural input from wearable earbuds to isolate the target speaker. 
To achieve real-time operation, we start with the Conv-TasNet source separation network~\cite{luo2019conv} and redesign the network to achieve a 90\% re-use of the computed network activations from the previous time step for each new audio segment (see~\xref{sec:nn}). While these optimizations make this network real-time, they also introduce artifacts in the audio output. To address this, we combine our mobile temporal model with a real-time  spectrogram-based frequency masking neural network. We show that by combining the two networks and creating a light-weight cascaded  network,  we can reduce artifacts and improve the audio quality further. {We present a training methodology that uses both synthetic data and small amounts of hardware data (see~\xref{sec:datasets}) 
to create a neural network that generalizes to  users and multi-path environments not in the training data. } \squishend

\begin{figure}[t]
\vskip -0.1in
\centering
\includegraphics[width=1\linewidth]{figures/side_voice_figure_v3.png}
\vskip -0.15in
\caption{\footnotesize{Background voice performance. { We use spatial cues to  separate background voices from the target speaker, even when the background voice is louder than the target voice. This is evident when the target speaker is silent  but background voice continues to talk (highlighted in orange).  Apple AirPods Pro  uses an endfire beamformer to partially suppress  background voice. The mono-channel Facebook Denoiser (Demucs) is unable to suppress the background voice. Clearbud's network  removes the background voice, approaching  ground truth. Comparing with Airpods:  \textcolor{blue}{\url{https://youtu.be/j8P2Q-PkuII}} }}}
\label{fig:fig3}
\vskip -0.2in
\end{figure}

We combine our wireless earbuds and neural network to create ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time, on-device processing on a commodity mobile phone paired to the  two earbuds.  Our results show that:
\squishlist
    \item Our binaural wireless earbuds  can stream audio to a phone with a synchronization error less than 64$\mu$s and operate  continuously on a coin cell battery for 40 hours.
    \item Our system outperforms Apple AirPods Pro by 5.23, 8.61, and 6.94~dB  for the tasks of  separating the target voice from background noise, background voices, and a combination of background noise and voices respectively.
    \item Our network has a runtime of 21.4ms on iPhone 12, and the entire ClearBuds system operates in real-time with an end-to-end  latency of 109ms.  For telephony applications, an ear-to-mouth latency of less than 200ms is required for a good user experience \cite{g.114}.
    \item In-the-wild evaluation with eight users in various indoor and outdoor scenarios  shows that our system  generalizes to previously unseen participants and multipath environments,  that are not in the training data.  
    \item In a user study with 37  participants who spent over 15.4  hours and rated a total of 1041  in-the-wild  audio samples, our cascaded network achieved a higher mean opinion score and noise suppression  than both the input speech as well as a  lightweight Conv-TasNet network. 
    
    
%    \item Our network can run in real-time on a mobile device with a latency of 155ms on an iPhone 12
\squishend




We believe that this paper  bridges state-of-the-art deep  learning for blind audio source separation and in-ear mobile systems. The ability to perform background noise suppression and   speech  separation could positively   impact  millions of people who use earbuds to take calls on-the-go. By open-sourcing the hardware  and collected datasets, our work may  help kickstart future research among mobile system and machine learning researchers to design  algorithms around wireless earbud data.

    
    
    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Imagine a world a in 

% They cannot do two channel because of bluetooth reasons

% They are doing beamforming on one device

% What is the first thing that we're doing

% What's novel about the end to end system, it's real time, on the mobile device, using two mics

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Background noise during phone and video calls is a persistent problem that affects people all over the world. Environmental sounds, such as street noises, machinery noises, or other people talking, can be transmitted along with the speaker, which hinders the ability to clearly communicate.

% Speech enhancement is the task of isolating the speaker of interest and suppressing all unwanted background sounds. Recently, there have been many advances in machine learning that attempt to remove these artifacts from a single microphone input. Such systems do not perform well in situations where multiple human speakers are present due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker. In addition, such systems generally perform worse than those that utilize multiple microphones.  

%  We are particularly motivated by the rise in multi-microphone wearable headphones in everyday settings. Examples include AirPods and PixelBuds, which have become increasingly popular in recent years. Although these devices often employ some amount of directional pickup, via beamforming or microphone design, these mechanisms offer limited attenuation of background noise compared to deep learning methods.
 
%  In contrast to these approaches, we propose a neural network that utilizes binaural input from wearable headphones in order to isolate the target speaker based on both voice and spatial information. Furthermore, we design our network to run real-time on a mobile device and show low latency across a variety of devices. To achieve real-time separation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 50ms, we can re-use 99\% of the computed network activations from the previous time step for each new segment of audio. Experiments show that our network can outperform a number of baselines on both synthetic and real data.
 
%  As a further contribution, we designed a set of wireless earbuds that maintain time synchronization between the microphones at a resolution of 32 microseconds. We built a custom wireless protocol over Bluetooth Low Energy (BLE) to enable synchronized, two-channel microphone streaming to the mobile device. To our knowledge, this is one of the first systems to be able to synchronously stream each microphone channel from each earbud to the mobile phone. This represents a step forward from single earbud beam-forming techniques, which were designed around the fact that current Bluetooth audio protocols only support one microphone channel for uplink. We expect our wireless earbuds to be of wider interest to the spatial audio community as a research and development platform.
 
% %  Because the current Bluetooth hands-free profile (HFP) only supports one microphone for uplink, 
 
% %  This represents a step forward from traditional single-side, on-device beam-forming techniques, and we expect our technique to be of wider interest to the spatial audio community.
 
%  We combine the neural network with our headphones to create a system called ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%

% For most use cases, speech enhancement systems must run in real-time on the hardware available. This hardware includes both the microphone available as well as the processing hardware. Although many previous works use a single microphone along with a GPU or a laptop CPU,


% In contrast to traditional speech enhancement techniques, we notice that the geometry of the mouth with respect to earbuds allows us to apply an additional geometric heuristic, which then allows us to adapt source separation techniques to speech enhancement. xxxxxx

% In contrast to more general purpose source separation formulations, the key insight is that for speech enhancement on wireless earbuds, the goal is to focus on the voice source  that is approximately equidistant from the two earbuds. 

% To separate the wearer's voice we train a neural network to separate voice sources that are in the center of the microphone array. We use a similar technique as Cone-of-Silence, but do not need the location conditioning variables because the target speaker is always in a known position. xr

% P1
% (1) Succinctly define the problem. Need speech enhancement on earbuds. Focusing on the person who is talking.
% (2) This is useful because people are talking while walking around (buses, streets) with wireless earbuds, existing approaches are not equipped to solve this.

% P2
% Beamforming, why they don't work. 2-3 academic citations, limited because of this reason. 
% On the other hand neural networks have done single channel, but they are limited due to .
% Synthetic data , non causal

% P3
% We built xxx. Key insight to make this realtime is xx. Built system which can wirelessly stream this thing and collected real data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textcolor{red}{Shyam: This history lesson is not required.}
%  In all aspects of our daily lives, the ability for us to hold conversations from one to another anywhere around the world has become an ability that is important in both our personal and work lives. Engineering efforts continue to push the telephony experience by improving voice quality, reducing latency, and eliminating background noise for a better experience. Finally, the advent of telephony has also contributed toward the rapid advancement of audio devices such as wireless earbuds and headsets for both improved voice quality and the ability to take calls hands-free.

% % Improvements in the telephony experience also extend into the video domain. Video calls and video conferencing have been established so that we can now see each other’s faces to further improve the experience of effectiveness of our ability to communicate and collaborate with each other. In the work environment especially, video conferencing has become a necessity for employees and collaborators working from home and working remotely. Indeed, the SARS-CoV-2 (COVID-19) pandemic has only exacerbated this need, as the need for effective video conferencing software (Zoom, Microsoft Teams, Cisco Webex) has become a staple for us to remain effective while we work from home.

% \textcolor{red}{In efforts to continue to improve the telephony experience, engineering innovations are made across both the hardware and software space. For example, digital MEMS microphones have long been preferred to their analog counterparts for noise immunity in wireless audio systems with high frequency radio components.} Today’s phones and wireless earbuds have also taken a step further by adding beam-forming to amplify a speaker’s voice while attenuating external background noise. While the strengths of beam-forming become stronger with distance between two microphones, companies like Apple and Google still integrate dual microphones on their wireless earbuds like AirPods and PixelBuds to gain the benefits of beam-forming microphones. While beam-forming functions well on these edge devices, its ability to attenuate non-broadband-noise fall short. Noises such as loud buses and subways, home appliances, and other background voices persist in the audio uplink during a voice call, disrupting the overall communication experience.

% Recently, developments in the machine learning space have attempted to remove these extremities from a single microphone channel. These networks operate by utilizing spectrogram transformations to learn human voice priors, thus retaining human speech while eliminating other noises. While research continues in the academic space, companies like Krisp have begun to productize this technology so that people can enjoy voice and video calls with background noise removal in the uplink channel. Interest in this technology has also influenced companies like Google, as they recently introduced background noise cancellation on their video conferencing platform, Google Meet.

% While Krisp and Google Meet perform well to isolate human speakers while eliminating background noise, they do not perform well in situations where multiple human speakers are present. This is primarily due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker in respect to surrounding background voices. This is a nontrivial pitfall, as the ability for these networks to remove noise and background voices in environments such as cafes, call centers, or shared work spaces become weaker.

% To combat this, we introduce and propose ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. The basis of our contributions function by integrating both the advances in the wireless earbud ecosystem along with audio source separation networks in the deep learning space. Specifically, we architect and engineer a solution which streams microphone data from both a user’s left and right ear as inputs for our source separation network. With two input channels, our network now attains the spatial information required to eliminate background voices while also isolating the intended speaker, which should be spatially equidistant between a pair of wireless earbuds.

% The contributions of this approach are feasible with our end-to-end system which consists of a pair of wireless earbuds and a mobile phone. Custom firmware is embedded in each earbud which maintains time synchronization between the microphones at a resolution of 32 microseconds. Additionally, a custom wireless protocol is designed to stream the time-synced microphones in real-time to a mobile phone for processing. To our knowledge, this is the first system in which multiple wireless microphones are leveraged to expand upon commercially available background noise cancellation voice technologies (Krisp, Google Meet). Transitively, this is also the first demonstration of streaming both microphones in a pair of wireless earbuds, taking a step forward from traditional single-side, on-device beam-forming techniques. We present comparative results to show that we perform comparatively against non-causal [deep learning model] by xxx dB, while outperforming commercially available models (Krisp) by xxx dB and on-device beam-forming (AirPods) by xxx dB. 


==> sections/1-intro-5.tex <==
\section{Introduction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 5 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With the rapid proliferation of wireless earbuds (100 million AirPods sold in 2020~\cite{airpodssales}), more people than ever are taking calls on-the-go.  While these systems offer unprecedented convenience, their mobility raises an important technical challenge:  environmental noise (e.g., street sounds, people talking)  can interfere and make it harder to understand the speaker.
We therefore seek to enhance the speaker's voice, and suppress background sounds using speech captured across the two earbuds. 

Source separation of acoustic signals is a long-standing problem where the conventional approach for decades has been to perform beamforming using multiple microphones. Signal processing-based beamformers that are computationally light-weight can encode the spatial information  but do not effectively capture the acoustic cues~\cite{van1988beamforming,krim1996two,chhetri2018multichannel}.
Therefore, the ability of the system to separate the user’s voice is limited, resulting in bleed through of environmental sounds and voices, as can be seen in Fig. \ref{fig:fig3} and heard in the AirPods section of the video demo.
Deep neural networks have been shown to be  more effective at suppressing a range of interfering audio sources with recent work demonstrating gains of up to $9$~dB over signal processing baselines in source separation tasks ~\cite{subakan2021attention,luo2019conv}. \textcolor{red}{However, taking these architectures and directly deploying them in a mobile earbud environment is challenging for two reasons.
First, the computational footprint of these high-performance neural networks can be many times that of a beamformer. Therefore, even real-time implementations of such networks are run on cloud~\cite{krisp} or require desktop GPUs [add citation] with privacy and cost implications. Performance drops as resource and latency constraints are applied, especially under severe constraints such as those associated with running real-time on a mobile device.
Second, these neural network systems learn acoustic cues, recognizing the sound signature of the class of target source (human voice) and interfering sources (everything else). When deployed in real environments, these networks let other background voices pass through, especially when the target speaker is not speaking (see Fig. \ref{fig:fig3}).}

\textcolor{red}{We notice the unique spatial configuration of worn earbuds -- two microphones on either side of the target speaker's mouth -- offers an additional mode of separation. If if it is possible deploy a \textit{dual-channel} deep network on a pair of earbuds, one could exploit this unique placement, and can utilize \textit{both} spatial and acoustic cues simultaneously, resulting in better performance especially in the presence of background voices.}

\textcolor{red}{To realize this vision, there are three fundamental issues that must be addressed together to deliver a functioning, practical system:}
\begin{enumerate}
    \item Today's wireless earbuds only support one channel of microphone up-link to the phone. AirPods and similar devices upload microphone output from only a single earbud at a time.  To achieve binaural speaker separation, we need to design and build novel earbud hardware that can synchronously transmit audio data from both the earbuds, and maintain tight synchronization over long periods of time.
    \item Binaural speech enhancement networks are not lightweight and have not been demonstrated with wireless earbuds. Reducing the network size naively often leads to unpleasant artifacts. Thus, we also need to optimize the neural networks to run in real-time on smart devices that have a limited computational capability compared to cloud GPUs. Further, we need to meet the end-to-end latency requirements for telephony applications and ensure that the resulting audio output has a high quality from a user experience perspective.
    \item Prior binaural speech enhancement networks are trained and tested on synthetic data and have not been shown to generalize well to real data. Building an end-to-end system however requires a network that generalizes to in-the-wild real use. 
\end{enumerate}
    

\begin{figure}[t!]
\centering
 \includegraphics[width=1\linewidth]{figures/flow-diagram-6.png}
\vskip -0.1in
\caption{\footnotesize{ ClearBuds Application.  Our goal is to isolate a user's voice from background noise (e.g., street sounds or other people talking) by performing source separation  using a pair of custom designed, synchronized, wireless earbuds.}}
\label{fig:block_diagram}
\vskip -0.15in
\end{figure}

In this paper, we present the first system that uses neural networks to achieve real-time speech enhancement from binaural wireless earbuds.
Our key insight is to treat wireless earbuds as a binaural microphone array,
and exploit the specific geometry -- two well-separated microphones behind a proximal source -- to devise a specialized neural network for high quality speaker separation. In contrast to using multiple microphones on the same earbud to perform beamforming, as is common in wireless earbuds (e.g., Apple Airpods \cite{airpods}) and hearing aids, we use microphones across the left and right earbuds, increasing the distance between the two microphones and thus the spatial resolution. 

To achieve this system, we make two contributions spanning earable hardware and neural networks. 

\begin{figure}[t!]
\vskip -0.1in
\centering
\includegraphics[width=1\linewidth]{figures/clearbuds.png}
\vskip -0.15in
\caption{\footnotesize{ClearBuds hardware. The images show ClearBuds  inside 3D-printed enclosure and when  placed beside a quarter. }}
\label{fig:earbuds}
\vskip -0.15in
\end{figure}

\squishlist
\item {\bf Synchronized  binaural earables.} We designed a binaural wireless earbud system  (Fig.~\ref{fig:earbuds}) 
capable of streaming two time-synchronized microphone audio streams to a mobile device. This is one of the first systems of its kind, and we expect our earbud hardware and firmware (open-sourced at publication) to be of wider interest as a research and development platform. Existing earable platforms such as eSense~\cite{esense-1}  do not support time-synchronized audio transmission from two earbuds to a mobile device. 
We designed our DIY hardware  using open source eCAD software, outsourced fabrication and assembly to PCBWay ($\$2$K for 50 units), and 3D printed the  enclosures.

\item {\bf Light-weight cascaded neural network.} We introduce a light-weight  neural network  that utilizes binaural input from wearable earbuds to isolate the target speaker. 
To achieve real-time operation, we start with the Conv-TasNet source separation network~\cite{luo2019conv} and redesign the network to achieve a 90\% re-use of the computed network activations from the previous time step for each new audio segment (see~\xref{sec:nn}). While these optimizations make this network real-time, they also introduce artifacts in the audio output. To address this, we combine our mobile temporal model with a real-time  spectrogram-based frequency masking neural network. We show that by combining the two networks and creating a light-weight cascaded  network,  we can reduce artifacts and improve the audio quality further. {We present a training methodology that uses both synthetic data and small amounts of hardware data (see~\xref{sec:datasets}) 
to create a neural network that generalizes to  users and multi-path environments not in the training data. } \squishend

\begin{figure}[t]
\vskip -0.1in
\centering
\includegraphics[width=1\linewidth]{figures/side_voice_figure_v3.png}
\vskip -0.15in
\caption{\footnotesize{Background voice performance. { We use spatial cues to  separate background voices from the target speaker, even when the background voice is louder than the target voice. This is evident when the target speaker is silent  but background voice continues to talk (highlighted in orange).  Apple AirPods Pro  uses an endfire beamformer to partially suppress  background voice. The mono-channel Facebook Denoiser (Demucs) is unable to suppress the background voice. Clearbud's network  removes the background voice, approaching  ground truth. Comparing with Airpods:  \textcolor{blue}{\url{https://youtu.be/j8P2Q-PkuII}} }}}
\label{fig:fig3}
\vskip -0.2in
\end{figure}

We combine our wireless earbuds and neural network to create ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time, on-device processing on a commodity mobile phone paired to the  two earbuds.  Our results show that:
\squishlist
    \item Our binaural wireless earbuds  can stream audio to a phone with a synchronization error less than 64$\mu$s and operate  continuously on a coin cell battery for 40 hours.
    \item Our system outperforms Apple AirPods Pro by 5.23, 8.61, and 6.94~dB  for the tasks of  separating the target voice from background noise, background voices, and a combination of background noise and voices respectively.
    \item Our network has a runtime of 21.4ms on iPhone 12, and the entire ClearBuds system operates in real-time with an end-to-end  latency of 109ms.  For telephony applications, an ear-to-mouth latency of less than 200ms is required for a good user experience \cite{g.114}.
    \item In-the-wild evaluation with eight users in various indoor and outdoor scenarios  shows that our system  generalizes to previously unseen participants and multipath environments,  that are not in the training data.  
    \item In a user study with 37  participants who spent over 15.4  hours and rated a total of 1041  in-the-wild  audio samples, our cascaded network achieved a higher mean opinion score and noise suppression  than both the input speech as well as a  lightweight Conv-TasNet network. 
    
    
%    \item Our network can run in real-time on a mobile device with a latency of 155ms on an iPhone 12
\squishend




In this paper, we look to  bridge state-of-the-art deep learning for blind audio source separation and in-ear mobile systems. The ability to perform background noise suppression and   speech  separation could benefit  millions of people who use earbuds to take calls on-the-go. By open-sourcing the hardware, firmware, and neural network, we hope our work will  help to kickstart future research among mobile system and machine learning researchers to design  algorithms around wireless earbud data.

    
    
    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Imagine a world a in 

% They cannot do two channel because of bluetooth reasons

% They are doing beamforming on one device

% What is the first thing that we're doing

% What's novel about the end to end system, it's real time, on the mobile device, using two mics

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Background noise during phone and video calls is a persistent problem that affects people all over the world. Environmental sounds, such as street noises, machinery noises, or other people talking, can be transmitted along with the speaker, which hinders the ability to clearly communicate.

% Speech enhancement is the task of isolating the speaker of interest and suppressing all unwanted background sounds. Recently, there have been many advances in machine learning that attempt to remove these artifacts from a single microphone input. Such systems do not perform well in situations where multiple human speakers are present due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker. In addition, such systems generally perform worse than those that utilize multiple microphones.  

%  We are particularly motivated by the rise in multi-microphone wearable headphones in everyday settings. Examples include AirPods and PixelBuds, which have become increasingly popular in recent years. Although these devices often employ some amount of directional pickup, via beamforming or microphone design, these mechanisms offer limited attenuation of background noise compared to deep learning methods.
 
%  In contrast to these approaches, we propose a neural network that utilizes binaural input from wearable headphones in order to isolate the target speaker based on both voice and spatial information. Furthermore, we design our network to run real-time on a mobile device and show low latency across a variety of devices. To achieve real-time separation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 50ms, we can re-use 99\% of the computed network activations from the previous time step for each new segment of audio. Experiments show that our network can outperform a number of baselines on both synthetic and real data.
 
%  As a further contribution, we designed a set of wireless earbuds that maintain time synchronization between the microphones at a resolution of 32 microseconds. We built a custom wireless protocol over Bluetooth Low Energy (BLE) to enable synchronized, two-channel microphone streaming to the mobile device. To our knowledge, this is one of the first systems to be able to synchronously stream each microphone channel from each earbud to the mobile phone. This represents a step forward from single earbud beam-forming techniques, which were designed around the fact that current Bluetooth audio protocols only support one microphone channel for uplink. We expect our wireless earbuds to be of wider interest to the spatial audio community as a research and development platform.
 
% %  Because the current Bluetooth hands-free profile (HFP) only supports one microphone for uplink, 
 
% %  This represents a step forward from traditional single-side, on-device beam-forming techniques, and we expect our technique to be of wider interest to the spatial audio community.
 
%  We combine the neural network with our headphones to create a system called ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%

% For most use cases, speech enhancement systems must run in real-time on the hardware available. This hardware includes both the microphone available as well as the processing hardware. Although many previous works use a single microphone along with a GPU or a laptop CPU,


% In contrast to traditional speech enhancement techniques, we notice that the geometry of the mouth with respect to earbuds allows us to apply an additional geometric heuristic, which then allows us to adapt source separation techniques to speech enhancement. xxxxxx

% In contrast to more general purpose source separation formulations, the key insight is that for speech enhancement on wireless earbuds, the goal is to focus on the voice source  that is approximately equidistant from the two earbuds. 

% To separate the wearer's voice we train a neural network to separate voice sources that are in the center of the microphone array. We use a similar technique as Cone-of-Silence, but do not need the location conditioning variables because the target speaker is always in a known position. xr

% P1
% (1) Succinctly define the problem. Need speech enhancement on earbuds. Focusing on the person who is talking.
% (2) This is useful because people are talking while walking around (buses, streets) with wireless earbuds, existing approaches are not equipped to solve this.

% P2
% Beamforming, why they don't work. 2-3 academic citations, limited because of this reason. 
% On the other hand neural networks have done single channel, but they are limited due to .
% Synthetic data , non causal

% P3
% We built xxx. Key insight to make this realtime is xx. Built system which can wirelessly stream this thing and collected real data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textcolor{red}{Shyam: This history lesson is not required.}
%  In all aspects of our daily lives, the ability for us to hold conversations from one to another anywhere around the world has become an ability that is important in both our personal and work lives. Engineering efforts continue to push the telephony experience by improving voice quality, reducing latency, and eliminating background noise for a better experience. Finally, the advent of telephony has also contributed toward the rapid advancement of audio devices such as wireless earbuds and headsets for both improved voice quality and the ability to take calls hands-free.

% % Improvements in the telephony experience also extend into the video domain. Video calls and video conferencing have been established so that we can now see each other’s faces to further improve the experience of effectiveness of our ability to communicate and collaborate with each other. In the work environment especially, video conferencing has become a necessity for employees and collaborators working from home and working remotely. Indeed, the SARS-CoV-2 (COVID-19) pandemic has only exacerbated this need, as the need for effective video conferencing software (Zoom, Microsoft Teams, Cisco Webex) has become a staple for us to remain effective while we work from home.

% \textcolor{red}{In efforts to continue to improve the telephony experience, engineering innovations are made across both the hardware and software space. For example, digital MEMS microphones have long been preferred to their analog counterparts for noise immunity in wireless audio systems with high frequency radio components.} Today’s phones and wireless earbuds have also taken a step further by adding beam-forming to amplify a speaker’s voice while attenuating external background noise. While the strengths of beam-forming become stronger with distance between two microphones, companies like Apple and Google still integrate dual microphones on their wireless earbuds like AirPods and PixelBuds to gain the benefits of beam-forming microphones. While beam-forming functions well on these edge devices, its ability to attenuate non-broadband-noise fall short. Noises such as loud buses and subways, home appliances, and other background voices persist in the audio uplink during a voice call, disrupting the overall communication experience.

% Recently, developments in the machine learning space have attempted to remove these extremities from a single microphone channel. These networks operate by utilizing spectrogram transformations to learn human voice priors, thus retaining human speech while eliminating other noises. While research continues in the academic space, companies like Krisp have begun to productize this technology so that people can enjoy voice and video calls with background noise removal in the uplink channel. Interest in this technology has also influenced companies like Google, as they recently introduced background noise cancellation on their video conferencing platform, Google Meet.

% While Krisp and Google Meet perform well to isolate human speakers while eliminating background noise, they do not perform well in situations where multiple human speakers are present. This is primarily due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker in respect to surrounding background voices. This is a nontrivial pitfall, as the ability for these networks to remove noise and background voices in environments such as cafes, call centers, or shared work spaces become weaker.

% To combat this, we introduce and propose ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. The basis of our contributions function by integrating both the advances in the wireless earbud ecosystem along with audio source separation networks in the deep learning space. Specifically, we architect and engineer a solution which streams microphone data from both a user’s left and right ear as inputs for our source separation network. With two input channels, our network now attains the spatial information required to eliminate background voices while also isolating the intended speaker, which should be spatially equidistant between a pair of wireless earbuds.

% The contributions of this approach are feasible with our end-to-end system which consists of a pair of wireless earbuds and a mobile phone. Custom firmware is embedded in each earbud which maintains time synchronization between the microphones at a resolution of 32 microseconds. Additionally, a custom wireless protocol is designed to stream the time-synced microphones in real-time to a mobile phone for processing. To our knowledge, this is the first system in which multiple wireless microphones are leveraged to expand upon commercially available background noise cancellation voice technologies (Krisp, Google Meet). Transitively, this is also the first demonstration of streaming both microphones in a pair of wireless earbuds, taking a step forward from traditional single-side, on-device beam-forming techniques. We present comparative results to show that we perform comparatively against non-causal [deep learning model] by xxx dB, while outperforming commercially available models (Krisp) by xxx dB and on-device beam-forming (AirPods) by xxx dB. 


==> sections/1-introduction.tex <==
\section{Introduction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%% SEE INTRO-2 %%%%%%%%%%%%%%%%%%%%%%%

% With the rapid proliferation of headsets and wireless earbuds, more people than ever are taking calls on-the-go. Apple Airpods alone have approximately doubled in sales each year since 2017 surpassing 100 million units sold in 2020.  While these systems offer unprecedented convenience, their mobility reveals another challenge: on a call, environmental sounds, such as street noises, machinery, or even other people talking, can be transmitted along with the speaker, hindering the ability to clearly communicate. To combat this background noise, wireless earbuds like Airpods use multiple microphones to beamform the mouth. Because Bluetooth HFP supports single-channel uplink and the fact that beamforming requires extremely low latency calculations on local DSPs, beamforming is performed using two microphones on a single earbud in an end-fire configuration. This is where the conveniently small size of these devices become a double-edged sword: the extremely small baseline between microphones reduces beamforming gain allowing environmental noises to leak in. Furthermore, outside of being tuned to perform at a specific frequency, beamforming systems do not intelligently filter on the acoustic cues of a human voice.

% By learning these acoustic cues, deep learning methods have demonstrated promising speech enhancement performance. Typically, these algorithms perform on a single channel, however, such systems do not perform well in situations where multiple human speakers are present, since a single microphone model lacks the spatial information required to isolate the intended speaker. Recently, multi-channel source separation algorithms have shown impressive results isolating a target source via wired microphone arrays.
% %, but have typically been deployed on desktop and via post-processing.

% Our key insight is to treat binaural wireless earbuds as a microphone array that can filter the wearer's voice on both spatial information and acoustic speech cues. To realize our system, we designed a set of wireless earbuds that maintain time synchronization between the microphones at a resolution of 32 microseconds. We built a custom wireless protocol over Bluetooth Low Energy (BLE) to enable synchronized, two-channel microphone streaming to the mobile device. To our knowledge, this is one of the first systems to be able to synchronously stream each microphone channel from each earbud to the mobile phone. We expect our wireless earbuds to be of wider interest to the spatial audio community as a research and development platform.

% We propose a neural network that utilizes binaural input from wearable headphones in order to isolate the target speaker based on both voice and spatial information. Furthermore, we design our network to run real-time on a mobile device and show low latency across a variety of devices. To achieve real-time separation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 50ms, we can re-use 99\% of the computed network activations from the previous time step for each new segment of audio. Experiments show that our network can outperform a number of baselines on both synthetic and real data.

% We combine our headphones and network to create a system called ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time, on-device processing on a commodity mobile phone paired to set of wireless earbuds. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Imagine a world a in 

% They cannot do two channel because of bluetooth reasons

% They are doing beamforming on one device

% What is the first thing that we're doing

% What's novel about the end to end system, it's real time, on the mobile device, using two mics

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Background noise during phone and video calls is a persistent problem that affects people all over the world. Environmental sounds, such as street noises, machinery noises, or other people talking, can be transmitted along with the speaker, which hinders the ability to clearly communicate.

% Speech enhancement is the task of isolating the speaker of interest and suppressing all unwanted background sounds. Recently, there have been many advances in machine learning that attempt to remove these artifacts from a single microphone input. Such systems do not perform well in situations where multiple human speakers are present due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker. In addition, such systems generally perform worse than those that utilize multiple microphones.  

%  We are particularly motivated by the rise in multi-microphone wearable headphones in everyday settings. Examples include AirPods and PixelBuds, which have become increasingly popular in recent years. Although these devices often employ some amount of directional pickup, via beamforming or microphone design, these mechanisms offer limited attenuation of background noise compared to deep learning methods.
 
%  In contrast to these approaches, we propose a neural network that utilizes binaural input from wearable headphones in order to isolate the target speaker based on both voice and spatial information. Furthermore, we design our network to run real-time on a mobile device and show low latency across a variety of devices. To achieve real-time separation, we use a Temporal Conv-Net based separation network that allows caching of intermediate outputs. When running on streaming input chunks of 50ms, we can re-use 99\% of the computed network activations from the previous time step for each new segment of audio. Experiments show that our network can outperform a number of baselines on both synthetic and real data.
 
%  As a further contribution, we designed a set of wireless earbuds that maintain time synchronization between the microphones at a resolution of 32 microseconds. We built a custom wireless protocol over Bluetooth Low Energy (BLE) to enable synchronized, two-channel microphone streaming to the mobile device. To our knowledge, this is one of the first systems to be able to synchronously stream each microphone channel from each earbud to the mobile phone. This represents a step forward from single earbud beam-forming techniques, which were designed around the fact that current Bluetooth audio protocols only support one microphone channel for uplink. We expect our wireless earbuds to be of wider interest to the spatial audio community as a research and development platform.
 
% %  Because the current Bluetooth hands-free profile (HFP) only supports one microphone for uplink, 
 
% %  This represents a step forward from traditional single-side, on-device beam-forming techniques, and we expect our technique to be of wider interest to the spatial audio community.
 
%  We combine the neural network with our headphones to create a system called ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%% RANDOM NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%

% For most use cases, speech enhancement systems must run in real-time on the hardware available. This hardware includes both the microphone available as well as the processing hardware. Although many previous works use a single microphone along with a GPU or a laptop CPU,


% In contrast to traditional speech enhancement techniques, we notice that the geometry of the mouth with respect to earbuds allows us to apply an additional geometric heuristic, which then allows us to adapt source separation techniques to speech enhancement. xxxxxx

% In contrast to more general purpose source separation formulations, the key insight is that for speech enhancement on wireless earbuds, the goal is to focus on the voice source  that is approximately equidistant from the two earbuds. 

% To separate the wearer's voice we train a neural network to separate voice sources that are in the center of the microphone array. We use a similar technique as Cone-of-Silence, but do not need the location conditioning variables because the target speaker is always in a known position. xr

% P1
% (1) Succinctly define the problem. Need speech enhancement on earbuds. Focusing on the person who is talking.
% (2) This is useful because people are talking while walking around (buses, streets) with wireless earbuds, existing approaches are not equipped to solve this.

% P2
% Beamforming, why they don't work. 2-3 academic citations, limited because of this reason. 
% On the other hand neural networks have done single channel, but they are limited due to .
% Synthetic data , non causal

% P3
% We built xxx. Key insight to make this realtime is xx. Built system which can wirelessly stream this thing and collected real data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DRAFT 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textcolor{red}{Shyam: This history lesson is not required.}
%  In all aspects of our daily lives, the ability for us to hold conversations from one to another anywhere around the world has become an ability that is important in both our personal and work lives. Engineering efforts continue to push the telephony experience by improving voice quality, reducing latency, and eliminating background noise for a better experience. Finally, the advent of telephony has also contributed toward the rapid advancement of audio devices such as wireless earbuds and headsets for both improved voice quality and the ability to take calls hands-free.

% % Improvements in the telephony experience also extend into the video domain. Video calls and video conferencing have been established so that we can now see each other’s faces to further improve the experience of effectiveness of our ability to communicate and collaborate with each other. In the work environment especially, video conferencing has become a necessity for employees and collaborators working from home and working remotely. Indeed, the SARS-CoV-2 (COVID-19) pandemic has only exacerbated this need, as the need for effective video conferencing software (Zoom, Microsoft Teams, Cisco Webex) has become a staple for us to remain effective while we work from home.

% \textcolor{red}{In efforts to continue to improve the telephony experience, engineering innovations are made across both the hardware and software space. For example, digital MEMS microphones have long been preferred to their analog counterparts for noise immunity in wireless audio systems with high frequency radio components.} Today’s phones and wireless earbuds have also taken a step further by adding beam-forming to amplify a speaker’s voice while attenuating external background noise. While the strengths of beam-forming become stronger with distance between two microphones, companies like Apple and Google still integrate dual microphones on their wireless earbuds like AirPods and PixelBuds to gain the benefits of beam-forming microphones. While beam-forming functions well on these edge devices, its ability to attenuate non-broadband-noise fall short. Noises such as loud buses and subways, home appliances, and other background voices persist in the audio uplink during a voice call, disrupting the overall communication experience.

% Recently, developments in the machine learning space have attempted to remove these extremities from a single microphone channel. These networks operate by utilizing spectrogram transformations to learn human voice priors, thus retaining human speech while eliminating other noises. While research continues in the academic space, companies like Krisp have begun to productize this technology so that people can enjoy voice and video calls with background noise removal in the uplink channel. Interest in this technology has also influenced companies like Google, as they recently introduced background noise cancellation on their video conferencing platform, Google Meet.

% While Krisp and Google Meet perform well to isolate human speakers while eliminating background noise, they do not perform well in situations where multiple human speakers are present. This is primarily due to the fact that a single microphone model lacks the spatial information required to isolate the intended speaker in respect to surrounding background voices. This is a nontrivial pitfall, as the ability for these networks to remove noise and background voices in environments such as cafes, call centers, or shared work spaces become weaker.

% To combat this, we introduce and propose ClearBuds, an end-to-end system capable of (1) source separation for the intended speaker in noisy environments, (2) attenuation and/or elimination of both background noises and external human voices, and (3) real-time processing on a pair of wireless earbuds paired with a mobile phone. The basis of our contributions function by integrating both the advances in the wireless earbud ecosystem along with audio source separation networks in the deep learning space. Specifically, we architect and engineer a solution which streams microphone data from both a user’s left and right ear as inputs for our source separation network. With two input channels, our network now attains the spatial information required to eliminate background voices while also isolating the intended speaker, which should be spatially equidistant between a pair of wireless earbuds.

% The contributions of this approach are feasible with our end-to-end system which consists of a pair of wireless earbuds and a mobile phone. Custom firmware is embedded in each earbud which maintains time synchronization between the microphones at a resolution of 32 microseconds. Additionally, a custom wireless protocol is designed to stream the time-synced microphones in real-time to a mobile phone for processing. To our knowledge, this is the first system in which multiple wireless microphones are leveraged to expand upon commercially available background noise cancellation voice technologies (Krisp, Google Meet). Transitively, this is also the first demonstration of streaming both microphones in a pair of wireless earbuds, taking a step forward from traditional single-side, on-device beam-forming techniques. We present comparative results to show that we perform comparatively against non-causal [deep learning model] by xxx dB, while outperforming commercially available models (Krisp) by xxx dB and on-device beam-forming (AirPods) by xxx dB. 

==> sections/2-related-1.tex <==
\section{Related Work}



%\begin{help-env}

Real-time speech enhancement is a long standing problem in the signal processing and machine learning communities.  While recent advances in the machine learning community have shown promising results, none of them have been demonstrated on wireless earbuds. Further, the vast majority cannot run on mobile devices and meet these real-time constraints. As a result, endfire beamforming configurations remain popular on most consumer mobile phones and earbuds \cite{samsungglobalnewsroom_2014, airpods, sennheiser_2020, beamforming-app-note}. Below, we briefly discuss beamforming, single channel speech enhancement networks, and binaural networks. By creating a wireless acoustic  network between two earbuds and a novel light-weight hybrid  time-domain and spectrogram-based  neural network, we show for the first time that real-time two-channel neural networks can outperform  current real-time speech enhancement approaches for wireless earbuds.

\vskip 0.05in\noindent{\bf Beamforming techniques.} A common approach to enhancing speech is to design a beamforming microphone array to be more sensitive to sounds coming from the direction of the user's mouth \cite{van1988beamforming} or voice~\cite{dov-uist21}. Since signal-processing based beamforming is computationally lightweight compared to other speech enhancement techniques, these techniques are deployed on many commercially available audio products today such as smart speakers \cite{amazon}, mobile phones \cite{samsungglobalnewsroom_2014}, and earbud devices like Apple AirPods \cite{airpods}. However, the performance of beamforming is limited by the geometry of the microphones and the distance between them \cite{van1988beamforming, InvenSense}. The form factor of devices like AirPods restricts both the number of microphones on a single earbud and the available distance between them, limiting the gain of the beamformer. While beamforming simultaneously across two earbuds could provide better performance in principle, current wireless architectures are limited to streaming from a single earbud at a time \cite{bluetooth}. Furthermore, adaptive beamformers such as MVDR \cite{frost1972MVDR}, while showing promise with relatively few interfering sources,  are sensitive to sensor placement tolerance and steering \cite{zhang2017deep, brandstein2001microphone}. Finally, beamforming leverages spatial cues only and does not use acoustic cues and perceptual differences to discriminate sources, information that machine learning methods leverage successfully.

% Don H. Johnson and Dan E. Dudgeon. Array Signal Processing: Concepts and Techniques. Simon & Schuster, Inc., USA, 1992

% Beamforming microphone arrays for speech enhancement, https://ieeexplore.ieee.org/abstract/document/225915

% Rate-Constrained Beamforming in Binaural Hearing Aids
% https://link.springer.com/content/pdf/10.1155/2009/257197.pdf

% Dual-Channel Speech Enhancement by
% Superdirective Beamforming
% https://link.springer.com/content/pdf/10.1155/ASP/2006/63297.pdf


%\vskip 0.05in\noindent{\bf Single-channel speech enhancement.} 
\vskip 0.05in\noindent{\bf Single-channel speech enhancement}
Recent deep learning techniques have led to significant progress in single channel speech enhancement methods. These models typically operate on spectrograms to separate the human voice from background noise \cite{realtimenoise, Mohammadiha_2013, online_nonnegative, nikzad2020deep, choi2019phaseaware, lstm_speechenhancement, fu2019metricgan, TFMasking}. However, recent trends have opted to operate directly on the time domain signals \cite{luo2019conv, germain2018speech, pascual2017segan, demucsreal, macartney2018improved}, yielding performance improvements over spectrogram approaches. Commercially available noise suppression software like Krisp \cite{krisp} and Google Meet \cite{googlemeet} have successfully deployed single-channel models in real-time and are available for use on mobile phones and desktop computers, processing is performed on the cloud. However, single-channel models can not effectively capture the spatial information and hence fail to isolate the intended speaker when there are multiple speakers present.

% --> some recent work on increasing performance to real-time applications
% Real Time Speech Enhancement in the Waveform Domain
% https://arxiv.org/abs/2006.12847

\vskip 0.05in\noindent{\bf Multi-channel source separation and speech enhancement}
%\subsection{Multi-channel source separation and speech enhancement}
Multi-channel methods have been shown to perform better than their single-channel source separation counterparts \cite{yoshioka2018multi, chen2018multi, zhang2017deep, gu2020enhancing, tzirakis2021multichannel, jenrungrot2020cone}. Binaural methods have also been used for source separation \cite{binaural1, han2020realtime, li2011two, reindl2010speech} and localization \cite{van2008binaural, lyon1983computational, kock1950binaural}. Our method improves on existing binaural methods by combining time-domain neural network with spectrogram-based frequency masking networks as well as optimizing them to enable   real-time processing on a phone. Recent works~\cite{binaural_osu, dual_phone} use multiple microphones on a smartphone for  speech-enhancement however neither of them demonstrates real-time performance of a smartphone. In contrast, we demonstrate the first system that achieves real-time speech enhancement using microphones on the two wireless earbuds. Further, as the distance between the earbuds is larger than the distance between microphones on a typical mobile phone, we can  attain a better baseline than a mobile phone implementation, while also retaining the ability to speak hands-free.

\vskip 0.05in\noindent{\bf  Earable computing and platforms}
There has been recent interest in earable computing and sensing~\cite{oesense21,esense-1,esense-2,plat-1,romit-1}. Earable platforms such as eSense~\cite{esense-1,esense-2} have enabled research in enabling various sensing applications using earable devices. eSense however does not support time-synchronized audio transmission from two earbuds to a mobile device. This is a critical requirement for achieving  speech enhancement using the  microphones on the two wireless earbuds.  OpenMHA~\cite{open-1,open-2} is a open signal processing {\it software} platform for hearing aid research. In contrast, we create wireless earbud hardware, which will be open-sourced at publication and can support synchronize wireless transmission from the two earbuds to achieve speech enhancement. 

% --> multi-mic
% Cone-of-silence

%Some approaches, such as \cite{binaural_osu, dual_phone} have used the multiple microphones on a smartphone for real-time speech-enhancement. However, these networks would have to be retrained for every mobile phone as the position and distance between these microphones could change with future iterations. As our method is instead deployed on wireless earbuds, the geometry of the speaker in respect to the microphones will remain consistent. Further, as the distance between the earbuds is larger than the distance between microphones on a typical mobile phone, we attain a better baseline than a mobile phone implementation, while also retaining the ability to speak hands-free.

% Orientation of phone
% Phone on speaker


% Xueliang Zhang and DeLiang Wang. Deep learning based binaural speech separation in reverberant environments. IEEE/ACM transactions on audio, speech, and language processing, 25(5):1075–1084, 2017.


% REAL-TIME SPEECH ENHANCEMENT USING AN EFFICIENT CONVOLUTIONAL RECURRENT NETWORK FOR DUAL-MICROPHONE MOBILE PHONES IN CLOSE-TALK SCENARIOS
% https://web.cse.ohio-state.edu/~wang.77/papers/TZW.icassp19.pdf


% REAL-TIME BINAURAL SPEECH SEPARATION WITH PRESERVED SPATIAL CUES
% https://arxiv.org/pdf/2002.06637.pdf


% REFS
% [1] Cone of Silence - https://arxiv.org/pdf/2010.06007.pdf

% [2] REAL-TIME SPEECH ENHANCEMENT USING AN EFFICIENT CONVOLUTIONAL
% RECURRENT NETWORK FOR DUAL-MICROPHONE MOBILE PHONES IN CLOSE-TALK
% SCENARIOS - https://web.cse.ohio-state.edu/~wang.77/papers/TZW.icassp19.pdf

% [3] REAL-TIME SPEECH ENHANCEMENT USING EQUILIBRIATED RNN - https://arxiv.org/pdf/2002.05843.pdf

% [4] Real Time Speech Enhancement in the Waveform Domain - https://arxiv.org/pdf/2006.12847.pdf

% [5] https://developer.nvidia.com/blog/nvidia-real-time-noise-suppression-deep-learning/

% [6] https://dl.acm.org/doi/10.1109/TASLP.2014.2364452

% [7] Airpods https://support.apple.com/kb/SP750

% [8] Krisp https://krisp.ai/

% [9] An Experimental Study on Speech Enhancement
% Based on Deep Neural Networks https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=6665000

% [10] Subjective comparison and evaluation of speech enhancement algorithms https://www.sciencedirect.com/science/article/pii/S0167639306001920?casa_token=IKuQSbhWEN8AAAAA:IbDBcUaYbymPu2p0nY8qZ7-d2pTGsUwCf08HsBX4qvRVRX8C62PvqLPDnX_Ib7kFuaU3LXvsFA

% [11] Microphone Array Beamforming https://invensense.tdk.com/wp-content/uploads/2015/02/Microphone-Array-Beamforming.pdf

% [12] Beamforming microphone arrays for speech enhancement, https://ieeexplore.ieee.org/abstract/document/225915

% [13] Rate-Constrained Beamforming in Binaural Hearing Aids
% https://link.springer.com/content/pdf/10.1155/2009/257197.pdf

% [14] % Dual-Channel Speech Enhancement by
% Superdirective Beamforming
% https://link.springer.com/content/pdf/10.1155/ASP/2006/63297.pdf

% [15] Real Time Speech Enhancement in the Waveform Domain
% https://arxiv.org/abs/2006.12847

% [16] Xueliang Zhang and DeLiang Wang. Deep learning based binaural speech separation in reverberant environments. IEEE/ACM transactions on audio, speech, and language processing, 25(5):1075–1084, 2017.


% [17] REAL-TIME SPEECH ENHANCEMENT USING AN EFFICIENT CONVOLUTIONAL RECURRENT NETWORK FOR DUAL-MICROPHONE MOBILE PHONES IN CLOSE-TALK SCENARIOS
% https://web.cse.ohio-state.edu/~wang.77/papers/TZW.icassp19.pdf


% [18] REAL-TIME BINAURAL SPEECH SEPARATION WITH PRESERVED SPATIAL CUES
% https://arxiv.org/pdf/2002.06637.pdf

%\end{help-env}

==> sections/2-related.tex <==
\section{Related Work}

\begin{figure}[t!]
\vskip -0.1in
\centering
\includegraphics[width=0.75\linewidth]{figures/clearbuds.png}
\vskip -0.05in
\caption{\small{(Left) DIY  ClearBuds  inside 3D-printed enclosure. (Right) placed beside a quarter for scale. }}
\label{fig:earbuds}
\vskip -0.25in
\end{figure}

%\begin{help-env}

Real-time speech enhancement is a long standing problem in both the signal processing and machine learning communities. For telephony applications, an ear-to-mouth of less than 200ms is required for a good user experience \cite{g.114}. While recent advances in the machine learning community have shown promising results, the vast majority cannot run on mobile devices and meet these real-time constraints. As a result, endfire beamforming configurations remain popular on most consumer mobile phones and earbuds \cite{samsungglobalnewsroom_2014, airpods, sennheiser_2020, beamforming-app-note}. Below, we briefly discuss beamforming, single channel speech enhancement networks, and binaural networks. By creating a wireless acoustic sensor network between two earbuds, we show that our real-time two-channel neural network can outperform  current real-time speech enhancement approaches.

{\bf Beamforming techniques.} A common approach to enhancing speech is to design a beamforming microphone array to be more sensitive to sounds coming from the direction of the user's mouth \cite{van1988beamforming}. Since signal-processing based beamforming is computationally lightweight compared to other speech enhancement techniques, these techniques are deployed on many commercially available audio products today such as smart speakers \cite{amazon}, mobile phones \cite{samsungglobalnewsroom_2014}, and earbud devices like Apple AirPods \cite{airpods}. However, the performance of beamforming is limited by the geometry of the microphones and the distance between them \cite{van1988beamforming, InvenSense}. The form factor of devices like AirPods restricts both the number of microphones on a single earbud and the available distance between them, limiting the gain of the beamformer. While beamforming simultaneously from two earbuds could provide better performance in principle, current wireless architectures are limited to streaming from a single earbud at a time \cite{bluetooth}. Furthermore, adaptive beamformers such as MVDR \cite{frost1972MVDR}, while showing promise with relatively few interfering sources,  are sensitive to sensor placement tolerance and steering \cite{zhang2017deep, brandstein2001microphone}. Finally, beamforming does not use perceptual differences to discriminate sources, information that learning method leverage successfully.

% Don H. Johnson and Dan E. Dudgeon. Array Signal Processing: Concepts and Techniques. Simon & Schuster, Inc., USA, 1992

% Beamforming microphone arrays for speech enhancement, https://ieeexplore.ieee.org/abstract/document/225915

% Rate-Constrained Beamforming in Binaural Hearing Aids
% https://link.springer.com/content/pdf/10.1155/2009/257197.pdf

% Dual-Channel Speech Enhancement by
% Superdirective Beamforming
% https://link.springer.com/content/pdf/10.1155/ASP/2006/63297.pdf


{\bf Single-channel speech enhancement.} 
Recent deep learning techniques have led to significant progress in single channel speech enhancement methods. These models typically operate on spectrograms to separate the human voice from background noise \cite{realtimenoise, Mohammadiha_2013, online_nonnegative, nikzad2020deep, choi2019phaseaware, lstm_speechenhancement, fu2019metricgan, TFMasking}. However, recent trends have opted to operate directly on the waveforms in the time domain \cite{luo2019conv, germain2018speech, pascual2017segan, demucsreal, macartney2018improved} , yielding performance improvements over their frequency domain spectrogram counterparts. Commercially available noise suppression software like Krisp \cite{krisp} and Google Meet \cite{googlemeet} have successfully deployed these models in real-time and are available on mobile phones and desktop computers. However, single-channel models can not effectively capture the spatial information and hence  fail to isolate the intended speaker when there are multiple speakers present in the noisy channel.

% --> some recent work on increasing performance to real-time applications
% Real Time Speech Enhancement in the Waveform Domain
% https://arxiv.org/abs/2006.12847

{\bf Multi-channel source separation and speech enhancement.} Multi-channel methods have been shown to perform better than their single-channel source separation counterparts \cite{yoshioka2018multi, chen2018multi, zhang2017deep, gu2020enhancing, tzirakis2021multichannel, jenrungrot2020cone}. Binaural methods have also been used for source separation \cite{binaural1, han2020realtime, li2011two, reindl2010speech} and localization \cite{van2008binaural, lyon1983computational, kock1950binaural}. Our method improves on existing binaural methods by utilizing recent advances in waveform based source separation as well as by demonstrating real-time processing on a phone. 

% --> multi-mic
% Cone-of-silence

Some approaches, such as \cite{binaural_osu, dual_phone} have used the multiple microphones on a mobile device for real-time speech-enhancement. However, these networks would have to be retrained for every mobile phone as the position and distance between these microphones could change with future iterations. As our method is instead deployed on wireless earbuds, the geometry of the speaker in respect to the microphones will remain consistent. Further, as the distance between the earbuds is larger than the distance between microphones on a typical mobile phone, we attain a better baseline than a mobile phone implementation, while also retaining the ability to speak hands-free.

% Orientation of phone
% Phone on speaker


% Xueliang Zhang and DeLiang Wang. Deep learning based binaural speech separation in reverberant environments. IEEE/ACM transactions on audio, speech, and language processing, 25(5):1075–1084, 2017.


% REAL-TIME SPEECH ENHANCEMENT USING AN EFFICIENT CONVOLUTIONAL RECURRENT NETWORK FOR DUAL-MICROPHONE MOBILE PHONES IN CLOSE-TALK SCENARIOS
% https://web.cse.ohio-state.edu/~wang.77/papers/TZW.icassp19.pdf


% REAL-TIME BINAURAL SPEECH SEPARATION WITH PRESERVED SPATIAL CUES
% https://arxiv.org/pdf/2002.06637.pdf


% REFS
% [1] Cone of Silence - https://arxiv.org/pdf/2010.06007.pdf

% [2] REAL-TIME SPEECH ENHANCEMENT USING AN EFFICIENT CONVOLUTIONAL
% RECURRENT NETWORK FOR DUAL-MICROPHONE MOBILE PHONES IN CLOSE-TALK
% SCENARIOS - https://web.cse.ohio-state.edu/~wang.77/papers/TZW.icassp19.pdf

% [3] REAL-TIME SPEECH ENHANCEMENT USING EQUILIBRIATED RNN - https://arxiv.org/pdf/2002.05843.pdf

% [4] Real Time Speech Enhancement in the Waveform Domain - https://arxiv.org/pdf/2006.12847.pdf

% [5] https://developer.nvidia.com/blog/nvidia-real-time-noise-suppression-deep-learning/

% [6] https://dl.acm.org/doi/10.1109/TASLP.2014.2364452

% [7] Airpods https://support.apple.com/kb/SP750

% [8] Krisp https://krisp.ai/

% [9] An Experimental Study on Speech Enhancement
% Based on Deep Neural Networks https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=6665000

% [10] Subjective comparison and evaluation of speech enhancement algorithms https://www.sciencedirect.com/science/article/pii/S0167639306001920?casa_token=IKuQSbhWEN8AAAAA:IbDBcUaYbymPu2p0nY8qZ7-d2pTGsUwCf08HsBX4qvRVRX8C62PvqLPDnX_Ib7kFuaU3LXvsFA

% [11] Microphone Array Beamforming https://invensense.tdk.com/wp-content/uploads/2015/02/Microphone-Array-Beamforming.pdf

% [12] Beamforming microphone arrays for speech enhancement, https://ieeexplore.ieee.org/abstract/document/225915

% [13] Rate-Constrained Beamforming in Binaural Hearing Aids
% https://link.springer.com/content/pdf/10.1155/2009/257197.pdf

% [14] % Dual-Channel Speech Enhancement by
% Superdirective Beamforming
% https://link.springer.com/content/pdf/10.1155/ASP/2006/63297.pdf

% [15] Real Time Speech Enhancement in the Waveform Domain
% https://arxiv.org/abs/2006.12847

% [16] Xueliang Zhang and DeLiang Wang. Deep learning based binaural speech separation in reverberant environments. IEEE/ACM transactions on audio, speech, and language processing, 25(5):1075–1084, 2017.


% [17] REAL-TIME SPEECH ENHANCEMENT USING AN EFFICIENT CONVOLUTIONAL RECURRENT NETWORK FOR DUAL-MICROPHONE MOBILE PHONES IN CLOSE-TALK SCENARIOS
% https://web.cse.ohio-state.edu/~wang.77/papers/TZW.icassp19.pdf


% [18] REAL-TIME BINAURAL SPEECH SEPARATION WITH PRESERVED SPATIAL CUES
% https://arxiv.org/pdf/2002.06637.pdf

%\end{help-env}

==> sections/3-method.tex <==
\section{ClearBuds Design}

We first introduce our 
light-weight  neural network architecture that enables speech enhancement in real time for wireless earbuds. We then describe system design and physical specifications of our hardware platform and our synchronization algorithm to ensure time alignment between each ClearBud's microphone.

\begin{figure*}[t!]
\vskip -0.1in
\centering
\includegraphics[width=1\linewidth]{figures/network-diagram.png}
\caption{Network Diagram of CB-Net. Our network contains a time-domain component, shown in the top as CB-Conv-TasNet, and a frequency domain component, shown on the bottom by CB-UNet. The respective outputs are combined to produce the final output.}
\vskip -0.15in
\label{fig:network-full}
\end{figure*}


\subsection{Problem Formulation}
Suppose we have a 2 channel microphone array with one microphone on each ear of the wearer. The target voice is speaking with a signal $s_0 \in \mathbb{R}^{2 \times T}$ in the presence of some background noise $\textbf{bg}$ or other non-target speakers $s_{1..N}$. There may also be multi-path reflections and reverberations $\textbf{r}$ which we would also like to reduce.
\begin{equation}
    \mathbf{x} = \sum_{i=0}^{N}\mathbf{s}_i + \mathbf{bg} + \mathbf{r}.
\end{equation}
Our goal is then to recover the target speaker's signal, $s_{0}$, while ignoring the background, reverbations, or other speakers. We also must do so in a real-time way, meaning that the a mixture sample $\textbf{x}_t $ received at time $t$ must be processed and outputted by the network before $t + \textbf{L}$ for some defined latency $\textbf{L}$.  We refer to the non-target speakers as "background voices". These background voices may be at any location in the scene, including very close to the target speaker and their angle with respect to the speaker can change with time.



\subsection{Neural Network Architecture Motivation}\label{sec:nn}




We design a network that takes a binaural stream of audio and separates the target speaker. The network is  causal and runs in real-time on a mobile device. This is challenging for several reasons. First, the processing device has a much lower compute capacity, especially compared to standard GPUs. Additionally, the network needs to be able to separate background speakers as well as non-speech noises. To do this,  it must learn spatial cues in addition to voice characteristics. Finally, the resulting output should maximize the quality from a human experience perspective while minimizing any artifacts the network might introduce. 

Our network, which we call \textit{ClearBuds-Net} or \textit{CB-Net} for short, is a hybrid model that operates in both the time domain and frequency domain. The full network architecture is illustrated in Figure \ref{fig:network-full} and contains two main sub-components: A multi-channel time domain component called \textit{CB-Conv-TasNet}, and a frequency based component called \textit{CB-UNet}. In the following sections we first describe the motivation for each component of the network.


% \textcolor{red}{XXXThis needs to be rewritten. We need tos tart with the network architecutre and then talk about the details of each of the network and show example spectrograms to give the motivation for the frequency masking network.}


% To address this,. Second, the compute device has a much lower memory and compute capacity, especially compared to standard GPUs. To solve this, we use depthwise separable convolutions as described in \cite{howard2017mobilenets}. We also use a temporal convolution network (TCN) that allows caching of intermediate outputs to reduce computation on new packets. Finally, 


\subsubsection{CB-Conv-TasNet}
We base our time domain architecture on a multi-channel extension of Conv-TasNet \cite{luo2019conv}, a network in the waveform domain that has previously shown impressive results on the source separation problem. Conv-TasNet is lightweight, and its Temporal Convolution Network (TCN) structure lends itself to a causal implementation with intermediate layer caching \cite{paine2016fast}. We  use depthwise separable convolutions~\cite{howard2017mobilenets} to  further reduce the number of parameters and make the design real-time.   

A key feature of the time domain approach is that it can capture spatial cues in the network. In our design (Fig.~\ref{fig:block_diagram}), the desired source is always physically between  two  microphones, thus the voice signal will reach the microphones roughly at the same time. In contrast,  background or other speakers are typically not temporally aligned and will reach one microphone earlier or later. In \cite{jenrungrot2020cone}, it was shown that a time domain neural network can separate sources which are temporally aligned across the microphones while ignoring others. This is similar to a delay-and-sum beamforming effect, except the sum is replaced with a deep network. Since our proposed network also operates in the waveform domain we adapt the  spatial separation approach proposed in \cite{jenrungrot2020cone}  for our setup.


\subsubsection{CB-UNet}
Despite the strong performance of our lightweight CB-Conv-TasNet, the output often contains audible artifacts that reduce the listening experience. These artifacts have little effect on traditional metrics, like Signal-to-Distortion Ratio (SDR), but have a noticeable effect on subjective listening scores (see Sec.\ref{sec:mos}. These artifacts are often visible in a frequency representation of the audio. In Figure \ref{fig:spectrogram-motivation}, we show how the CB-Conv-TasNet alone contains noticeable artifacts when compared to the ground truth. To address this, we design and  implement a lightweight causal UNet \cite{ronneberger2015unet} which operates on the mel-scale spectrogram of the input audio. This network, which we call CB-UNet, produces a binary mask which is applied to the output of CB-Conv-TasNet. The combined output, shown in Figure \ref{fig:spectrogram-motivation} as CB-Net, is able to reduce these artifacts. The mean opinion scores in the experiment section further demonstrate the strength of the hybrid CB-Net when compared to the time-domain component only.

\begin{figure*}[t!]
%\vskip -0.1in
\centering
\includegraphics[width=1\linewidth]{figures/spectrogram_motivation.png}
\caption{The spectrograms above show the motivation behind a combined time and frequency domain method. The output of the time-domain component, CB-Conv-TasNet, contains artifacts, particularly at high frequencies. Although subtle, these artifacts are perceptible by human listeners. CB-Net is able to reduce these artifacts by using a frequency-domain network (CB-UNet) that masks unwanted frequencies.}
\label{fig:spectrogram-motivation}
\end{figure*}

\subsection{Neural Network Detailed Description}

In this section we describe the precise details of the full network architecture.

\subsubsection{CB-Conv-TasNet}
The input to the network is a binaural mixture given by $\textbf{x} \in \mathbb{R}^{2 \times T}$. The first step is an encoder that transforms the mixture $\textbf{x}$ into $\mathbb{R}^{N \times T/L}$ with a 1D convolution of size $L$ and stride $L$. This is followed by a ReLU layer. The encoder's outputs are next fed into a temporal convolution network that consists of stacks of 1-D convolutions with increasing dilation factors. We use 14 convolution layers with dilation factors of 1,2,4,..,64 repeated twice, with a ReLU nonlinearity and skip connection after each convolution. The encoder output is multiplied with the output of the temporal conv-net, before being fed through a fully connected Decoder layer which transforms the output back into $\mathbb{R}^{2 \times W}$. We describe window size  $W$ in the next sections. %\textcolor{red}{You can also refer to figure (need to insert) for a visual layout of the network.}


\begin{figure*}[t!]
\vskip -0.1in
\centering
\includegraphics[width=1\linewidth]{figures/network.png}
\vskip -0.15in
\caption{An illustration CB-Conv-TasNet, the time-domain component of CB-Net. Given a packet of 350 samples (22.4ms) highlighted in blue, we use \textasciitilde1.5 seconds of past input and 44.8ms of future input to output the separation results for this target packet. Our network is based on a temporal convolution network architecture with increasing dilation factors. Our caching scheme works as follows: When we receive a new 350ms samples, all the intermediate activations (circles in the diagram) slide to the left, and we only need to compute the rightmost column of outputs.}
\label{fig:network}
\vskip -0.2in
\end{figure*}

In a real-world implementation, we do not have access to the full waveform, but only packets of data at a time. Furthermore, we must process these packets with limited access to future input samples. Given  15.625 kHz sampling rate, we choose to process packets of 350 samples at a time (22.4ms), which we refer to as a window size $W$. We also use $2W$, or 700 samples of lookahead time (44.8ms) and \textasciitilde1.5s of past samples. Since we have no padding in the temporal convolution net, the network starts with this large temporal context and outputs exactly $\mathbb{R}^{1 \times W}$ samples, corresponding to the desired output for our input packet of $W$ samples. When we receive the next packet of size $W$, all intermediate activation from the encoder and temporal conv-net can be shifted over by $W / L$ samples and re-used. In our network we choose $L = 50$, but any divisor of $W$ would work. Re-using intermediate outputs from previous packets saves over $90\%$ of the compute time for a new packet in our network configuration. %These ideas of caching causal convolutions has been discussed in previous work such as \cite{paine2016fast}. %https://arxiv.org/pdf/1611.09482.pdf%


\subsubsection{CB-UNet}

The frequency domain network is a mono-channel network that outputs a binary mask for each time-frequency bin. The input $\textbf{x} \in \mathbb{R}^{1 \times T}$ is a summation of the binaural left and right channel, which is the equivalent of a broadside beamformer. We first run a STFT, which is a mel-scale fourier transform with hop size of $350$, a window size of  $1024$ including zero padding on the edges, and a $128$ bin mel-scale output. The network input is a spectrogram of $64$ time bins and $128$ frequency bins, corresponding to a receptive field of $22400$ samples, or $1.43s$. In order to maintain the causality requirement, we use the same lookahead strategy as the time-domain network where we allow $700$ samples of lookahead for a target packet of $350$ samples. The UNet architecture containes 4 downsampling and upsampling layers, starting with 64 channels and doubling the number of channels at each subsequent layer. The downsampling layers contain a depthwise separable convolution followed by a $2 \times 2$ max pooling, and the upsampling layers contain a depthwise separable convolution followed by a transposed convolution for upsampling. The output is a sigmoid function, which is then thresholded to return a binary mask in $[0, 1]^{128 \times 64}$. %Please refer to the original UNet paper for a detailed figure of the architecture.

When outputting a spectrogram mask on an $\mathbb{R}^{128 \times 64}$ input, we predict a mask over the entire input even though we only need the output for a specific slice of $350$ samples, or a $\mathbb{R}^{128 \times 1}$ mask. Further optimizations could be made by caching intermediate outputs or only computing the mask for the target samples. However the run-time of CB-UNet was so small compared to the rest of the network that we did not find these optimizations necessary.

\subsubsection{Combining the Outputs}
At each time step, the output of CB-Conv-Tasnet is an audio waveform in $x \in \mathbb{R}^{1 \times 350}$, and the output of CB-UNet is a spectrogram mask in $\textbf{M} \in \mathbb{R}^{128 \times 64}$. We run the same fourier transform on the buffered conv-tasnet outputs to produce a spectrogram $\textbf{X} \in \mathbb{R}^{128 \times 64}$. Our output can then be computed by $iSTFT(\textbf{M} \otimes \textbf{X})$.
 Our empirical results show that  this gives the best results compared to other methods such as ratio masking.
%Previous work \cite{zhao2018sound} has shown the benefits of binary masking for spectrogram based separation, and

\subsubsection{Training}
CB-Conv-TasNet is trained with an $L1$-based loss over the waveform along with the multi-resolution spectrogram loss. Formally, provided $s_{0}$ is our target speaker and $x'$ is the output from the network, our loss is:
\begin{equation}
    L(s_{0}, x') = \left\Vert s_{0} - x' \right\Vert_1 \\ + L_{sc}(s_0, x') + L_{mag}(s_0, x')
\end{equation}
\begin{equation}
L_{sc}(s_0, x') = \frac{\left\Vert STFT(s_0) - STFT(x')\right\Vert_F}{\left\Vert STFT(s_0)\right\Vert_F}
\end{equation}
\begin{equation}
L_{mag}(s_0, x') = \left\Vert \log(STFT(s_0) - \log(STFT(x'))  \right\Vert_1
\end{equation}
STFT denotes the magnitude of the short time Fourier transform, and $F$ denotes the Frobenius norm. $L_{sc}$ and $L_{mag}$ represent  spectral convergence and magnitude losses, which in our experience gave better results than L1 loss alone.

For training CB-UNet, for each time frequency bin, the training target $\textbf{M}$ is 1 if the target voice is the dominant component, and 0 otherwise. Formally, $\textbf{M}(f, t) = [\textbf{S}_{0}(f, t) \geq \textbf{S}_{i}(f, t)], \;\; \forall i = (1..n)$. The network is then trained with the binary cross entropy of the output compared to the target mask.

\subsection{Synchronized wireless earbuds}

\begin{figure*}[t!]
\vskip -0.1in
\centering
\includegraphics[width=0.9\linewidth]{figures/hardware-block-diagram.png}
\caption{Hardware Block Diagram (left), Custom Flex Circuit Board (top right), 3D-Printed Enclosures (bottom right). Each ClearBud integrates a PDM microphone, accelerometer, flash, and coin cell (CR2032) battery. Buttons and LEDs are used for interfacing with the device, and a USB port is used for programming and debug.}
\vskip -0.2in
\label{fig:sync}
\end{figure*}

\label{sec:system}
Our wireless earbud platform leverage both hardware and software components to achieve microphone synchronization between the two earbuds. We seek to capture speech from the target speaker's mouth which sits on the sagittal plane roughly  equidistant to the ears. Given an ear-to-ear spacing of 17.5cm, to effectively isolate this central plane we require a distance precision on the order of a few centimeters.
An interaural time difference of 100$\mu$s  would correspond to source maximally 3.43 cm off this central plane, therefore we target a synchronization accuracy under 100$\mu$s.

\subsubsection{Hardware} We develop wireless audio hardware capable of streaming time-synchronized microphones. Our architecture is a custom hardware design containing a %support for up to two 
pulse-density modulated (PDM) microphone (Invensense ICS-41350) and a Bluetooth Low Energy (BLE) microcontroller (Nordic nRF52840).\footnote{For future research applications, an ultra low-power accelerometer (Bosch BMA400), a 1Gbit NAND flash for local data collection (Winbond W25N01GVZEIG), and support for an additional microphone are included.} The system is powered off of a CR2032 coin cell battery and programmed via SWD over a Micro-USB connector.  Each ClearBud has an integrated PDM microphone set to a clock frequency of 2MHz. With an internal PDM decimation ratio of 64, this provides us a sampling frequency of 31.25kHz. As most HD voice applications and wideband codecs are limited to 16kHz~\cite{voicecodecs}, we decimate further in firmware by a factor of 2, giving us a final sampling frequency of 15.625kHz.
 Two 16-bit 180 sample size Pulse-Code Modulation (PCM) buffers are round-robined: one is filled with incoming PCM data while the other is processed. The DMA is responsible for both clocking in the PDM data and converting it into PCM. One buffer is always connected to the DMA, while the other is freed for processing for the rest of the data pipeline. When the buffer connected to the DMA fills, the buffers switch roles and we begin processing data on the newly freed buffer, and connect the other buffer back to the DMA. With this design we always have a continuous PCM stream to operate on.
Both ClearBuds transmit the PCM microphone data to a mobile phone for input into our neural network. To maximize throughput, we use the highest Bluetooth rate and packet sizes supported by iOS, which is 2Mbps and 182 bytes, respectively. We design a lightweight wireless protocol where the first 2 bytes represent a monotonically-increasing sequence number, while the other 180 bytes are reserved for the 16-bit PCM audio samples. The sequence number is used on the mobile phone so that we can zero-pad PCM data in the occasional event that a packet is dropped either over-the-air or at the radio hardware layer. This zero-padding keeps the left and right microphone streams aligned on the host side in areas of poor radio performance or interference.

\subsubsection{Fabrication} 
The hardware schematic and layout for ClearBuds was designed using the open source eCAD tool KiCad. A 2-layer flexible printed circuit were fabricated and assembled by PCBWay in China. The 3D printed enclosures were designed using AutoDesk Fusion 360 and printed with a Phrozen Sonic Mini ($\$340$) which uses a liquid resin fabrication process.   The MEMS microphone sits behind the lid on the earbud's outer surface facing outwards.
A single button on the enclosure to provide access to turn on and off the earbuds.

% The sequence number is used on the mobile phone so that we can zero-pad PCM data in the occasional event that a packet is dropped either over-the-air or at the radio hardware layer. This zero-padding keeps the left and right microphone streams aligned on the host side in areas of poor radio performance or interference. However, this is not sufficient to maintain synchronization within 100$\mu$s. We must also account for clock drift between our earbuds. MK: This sounds worse, as if this is the foundation for the sync and clock drift is the secondary feature.

% \begin{figure}[t!]
% \vskip -0.1in
% \centering
% \includegraphics[width=1\linewidth]{figures/hardware.png}
% \vskip -0.1in
% \caption{\small{Shio Hardware Architecture and Enclosure Design}}
% \label{fig:block_diagram}
% \vskip -0.1in
% \end{figure}

\begin{figure*}[t!]
\vskip -0.1in
\centering
\includegraphics[width=0.9\linewidth]{figures/mic-pipeline-2.png}
\caption{Time Sync Implementation. The primary ClearBud broadcasts a sync clock over the air. The secondary ClearBud then uses the sync clock to rate encode, by increasing or decreasing the size of its local PCM buffer. Both ClearBuds then decimate these buffers down by a factor of 2, and fill up a ring buffer. Finally, each BLE packet gets prepended with a sequence number and then gets transmitted to a host device. }
\label{fig:sync}
\end{figure*}

\begin{figure}
\centering     %%% not \center
\subfigure[]{\label{fig:sync-a}\includegraphics[width=0.23\textwidth]{figures/sync.png}}\hfill
\subfigure[]{\label{fig:sync-b}\includegraphics[width=0.23\textwidth]{figures/time-sync-cdf.png}}

\vskip -0.1in
\caption{Time Synchronization Validation. (a) Without time synchronization (red), microphone samples drift apart and lose alignment at about 128$\mu$s per minute. (b) CDF across three experiments of 5 minutes each. }
\label{fig:sync}
\vskip -0.2in
\end{figure}

%%Our system architecture revolves around the design of two microphones placed in each user's ear. We choose this design for two reasons. First, it allows us to leverage the spatial data of our desired voice being centered between the mics, while background noise has a higher likelihood of arriving off-center. Second, this configuration allows us to be directly applicable to devices in the hearable sector.

%One hurdle that needs to be overcome, is synchronizing the audio input from both wireless microphones so that our network can properly leverage the TDOA between the audio streams.

%  https://devzone.nordicsemi.com/nordic/short-range-guides/b/bluetooth-low-energy/posts/wireless-timer-synchronization-among-nrf5-devices


\subsubsection{Microphone synchronization} Three components are necessary for maintaining microphone synchronization between our two earbuds: (1) As each of our earbuds has its own local clock source, we need to establish a common clock between them so that they have the same reference of time, (2) a synchronized startup so each earbud starts recording from their respective microphone at the exact same time, and (3) a rate encoding scheme to control the earbud's sampling rate to match the other. 

In our system, each earbud has its own respective 32MHz clock source with a total +/- 20ppm frequency tolerance budget. So, in the worst case scenario, the earbuds will have 2.4 milliseconds of drift each minute. We  use the  Nordic's TimeSlot API \cite{timeslot}, which grants us access to the underlying radio hardware in between Bluetooth transmissions. This provides us a transport to transmit and receive accurate time sync beacons \cite{wireless-timesync}. Each ClearBud keeps a free-running 16MHz hardware timer with a max value of 800,000, overflowing and wrapping around at a rate of about 20~Hz. One ClearBud is assigned as the timing master while the other ClearBud will synchronize its respective free-running timer to the timing master (primary).  The primary ClearBud transmits time sync packets at a rate of 200~Hz. These packets contain the value of the free-running timer at the time of the radio packet transmission. When the secondary ClearBud receives this packet, it can then add or subtract an offset to its own free-running timer. This allows ClearBuds to maintain an accurate common clock. 

Once each ClearBud is connected to the mobile phone, the phone sends a \verb|START| command to both ClearBuds over BLE. Each ClearBud contains firmware which arms a programmable peripheral interconnect (PPI) to launch the PDM bus once the 16MHz free-running timer wraps around at 800,000. By using this method, we bypass the CPU and trigger a synchronized startup entirely at the hardware layer. One caveat is that the mobile phone could write to one ClearBud right \textit{before} its clock wraps around at 800,000, and the other ClearBud right \textit{after} it wraps around at 800,000. With a clock that wraps around at 20Hz, this would trigger a mismatched startup and cause an alignment error of 50ms. To correct for this, each ClearBud reports its common clock timer value to the phone once it has received the \verb|START| command. The phone can then remove the first 781 audio samples (781 samples / 15.625kHz = 50ms) if one ClearBud started streaming 50ms before the other.

The final component to keeping the audio streams aligned is to create a rate encoding scheme between the ClearBuds. With the time sync beacons from the primary ClearBud, the other ClearBud now has both its local clock and the common clock (primary ClearBud's local clock). With these two clocks, the secondary ClearBud can identify how much faster or slower its PDM clock is running in relation to the primary ClearBud. We note that with a 2MHz PDM clock and a PDM decimation ratio of 64, each audio sample occupies 32 microseconds. The non-primary ClearBud can then add or remove a sample to its PDM buffer every time the difference between the clocks exceeds a multiple of 32 microseconds. By doing this, the secondary ClearBud ensures that its PDM buffer starts filling up at the exact same time as the primary ClearBud's PDM buffer, with a tolerance of 32 us. 




\subsubsection{Hardware evaluation} In order to validate our synchronization firmware, we place both ClearBuds roughly equidistant from a speaker. A click tone is played every 15 seconds for 5 minutes, and recorded on both ClearBuds with time sync disabled and enabled. We calculate the sample error on each recorded click.
%, and convert it into time error with a sampling rate of 15.625kHz.
Figure ~\ref{fig:sync} shows the synchronization validation results across this experiment. We can see that with time sync enabled, the sample error never exceeds 1 sample at 15,625 kHz, or 64 $\mu$s.

Finally we evaluate the power consumption of the ClearBuds hardware. We measure current consumption by powering our system through its Micro-USB port with a power supply, which goes through the same power path as our coin cell battery. We set our power supply voltage to 3V and set a maximum current output of 300mA, to reflect the internal 10 ohm resistor of a CR2032 battery. While streaming microphone data, we measure current consumed to be between 5-6mA. With the CR2032's nominal capacity of 210mAh, this translates to 35-42 hours of streaming  operation.

%\begin{figure}[t!]
%\vskip -0.1in
%\centering
%\includegraphics[width=1\linewidth]{figures/mic-pipeline.png}
%\caption{\small{Microphone Data Pipeline}}
%\label{fig:mic_pipeline}
%\end{figure}

%[SHOW TIME SYNC PLOT]

%Two plots: Sine wave with time sync ON and sine wave with time sync OFF
%How to best represent drift on a graph? (5, 10, 15, 30, 60min?)

==> sections/4-OLDexperiments_and_results.tex <==
\section{Datasets and Training} \label{sec:datasets}
We train and evaluate the network on a variety of different datasets, including synthetic and real data. The datasets are described in the following sections.

Training and evaluating the network require clean ground truth speech samples as supervised learning targets. Therefore our data collection is based on the mix-and-separate framework \cite{zhao2018sound}, where clean speech and noise samples are recorded separately and combined randomly to form noisy mixtures. The network then learns to predict the clean speech given the noisy mixture. In order for this method of training to generalize to real scenarios, the recordings should mimic the dynamics of real speech as closely as possible, including reverb, voice resonance, and microphone response. Synthetically rendered spatial data is the easiest to obtain, but most different from real recordings, while real speakers wearing the headset in an anechoic chamber provide the best ground-truth, but are the most costly to obtain. Similar to \cite{jenrungrot2020cone}, we adopt a hybrid training structure where we first train on a large amount of synthetic data and fine-tune on real data recorded with our hardware. Our real demos and user studies show that this approach generalizes to naturally recorded noisy mixtures.

\subsection{Synthetic data} \label{sec:synthetic-data} To generate the synthetic dataset, we create multi-speaker recordings in simulated environments with reverb and background noises. Synthetic data is easily generated and can provide a wide variety of voice types and physical setups instantly. All voices come from the VCTK dataset \cite{vctk} (110 unique speakers), and background sounds come from the WHAM! dataset \cite{wham}, which contains 58 hours of recordings from a variety of noise environments such as a restaurant, crowd, ambient, street, and music.

 To synthesize a single example, we create a 3 second mixture as follows: two virtual microphones are placed 17.5~cm apart, which is the average distance between human ears \cite{RISOUD2018259}. The target speaker's voice is placed  at the center between the two virtual microphones, and a second voice is placed randomly between $1$ and $5$ meters away and at a random angle. A randomly chosen background noise is also placed in the scene. We then simulate room impulse responses (RIRs) for a randomly sized room using the image source method implemented in the pyroomacoustics library \cite{allen1979image, scheibler2018pyroomacoustics}. The room is rectangular with sides randomly chosen between 5 and 20 meters, and the RT60 values are randomly chosen between 0 and 1 second. All signals are convolved with the RIR and rendered to the two channel microphone array. The volumes of the background are randomly chosen so that the input signal-to-distortion ratio is roughly between -5 and 10dB. For training, we use 10,000 mixtures, and for testing we use 1,000. The train and test splits for both voice and background are independent, and there are no overlapping identities or samples.

% \textcolor{red}{XXXTHE ABOVE IS NOT A COMPLETE DISCRIPTION OF WHAT WAS DONE AND CANNOT BE USED TO REPLICATE. HERE IS AN EXAMPLE. To gather a large amount of training data, we use software to simulate random reverberate noisy rooms using the image source model~\cite{scheibler2018pyroomacoustics}. The rooms are simulated using absorption rates of real materials and a maximum RT60 of 500~ms. By default, we use a virtual 6-mic circular array with a radius of 5~cm. The distance between the virtual speakers and the microphone array is at least 0.8~m, and the direction of arrival differences of the speakers are at least $10^{\circ}$. The input direction is modeled as the groundtruth plus a random error less than $5^\circ$ simulating the gaze tracking measurement error \cite{sipatchin2020accuracy}.  We place virtual speakers at random locations within the room playing random speech utterances from the VCTK dataset~\cite{veaux2017cstr}, meanwhile simulating diffused noise from the MS-SNSD dataset~\cite{reddy2019scalable} and WHAM! dataset~\cite{wichern2019wham}. The combined speech power to noise ratio is randomized between $[5, 25]$~dB. 10\%, 40\%, 40\%, 10\% of the generated clips consists of 1-4 speakers, respectively, and we apply random gain within $[-5, 0]$~dB to each speaker. We guarantee that there exists speech utterance overlap for 2-4 speaker scenarios. We render the synthetic audio and generate 4s clips. We generate a total of 8000 clips as training set, 400 clips as validation set, and 200 clips as test set. No speech clips or noise has appeared in more than one of these three sets. }

\subsection{Hardware data} We also train and evaluate on a set of recorded samples from our ClearBuds prototypes. We set up a foam mannequin head with a speaker (Sony SBS-XB12) that plays VCTK samples. For clean speech recording, the speaker is placed in the position of the foam mannequin's mouth. For background voice recordings, the speaker is placed in varying locations within a one meter radius of the foam head. Real background noise is provided by binaural version of the WHAM! dataset \cite{wham}, which was recorded in real environments using a binaural mannequin like ours. For both training and testing, we record 2 hours each of clean speech, background noises, and background voices. 2000 random mixtures are created for both training and testing. We use a network pre-trained on synthetic data, and fine-tune it on the this recorded training data before evaluating on the test data.

%  When training, we randomly drop out the background noises and voices. In particular, each training example contains the target speaker all the time, and the background noise and background voice each with $70\%$ probability. This helps the network generalize to different background noise scenarios, including scenarios with no background noise or background voice. 


\begin{figure*}
\centering     
\subfigure[]{\label{}\includegraphics[width=0.35\textwidth]{figures/MOS_study_results_v2.png}}\hfill
\subfigure[]{\label{}\includegraphics[width=0.3\textwidth]{figures/user-study-indoors.jpg}}\hfill
\subfigure[]{\label{}\includegraphics[width=0.3\textwidth]{figures/user-study-outdoors.JPG}}\hfill
\vskip -0.15in
\caption{(a) Mean opinion score study results. Noise suppression indicates perceived quality of background noise reduction (higher is less intrusive). MOS indicates overall perceived quality (higher is preferred). Error bars are 95\% CI. For context, in the recent, flagship ICASSP 2021 Deep Suppression Noise Challenge \cite{icaasp_dns}, which consists of state-of-the-art, real-time algorithms run on a quad-core desktop CPU, the winning submission increased MOS by 0.57 opinion score points \cite{icaasp_dns_results}. (b,c) Example scenarios (cafe, street) of where user study samples were collected. User study samples were collected across 10 users and 5 environments, all unseen in our training dataset.}
\label{fig:mos-study-results}
\vskip -0.2in
\end{figure*}

\subsection{Real Data} To further generalize to real scenarios, we also collect a ground-truth speech dataset in an anechoic chamber with human speakers (5 male, 4 female) and an in-the-wild noise dataset from various environments. Each human speaker wore our ClearBuds prototypes, and uttered 15 minutes of text from Project Gutenberg in the anechoic chamber. The purpose of this anechoic data is to provide clean training targets for the network for speakers using our headset. The in-the-wild noise dataset was collected in various noisy scenarios such as vacuum cleaning, washing dishes, loud indoor/outdoor restaurants, and busy traffic intersections. 

% Finally, we collect an evaluation set with 2 human speakers (1 male, 1 female) in 2 noisy environments, both unseen and untrained on our network.  We also  provide  supplementary videos of the system being used in the wild in unseen locations and speakers.


\section{Experiments and Results}
We show several evaluations to demonstrate the strength of our method. First, we conduct a user study using completely in-the-wild recordings of a speaker in a noisy environment. Then we compare against AirPods using a repeatable audio setup that is run with both ClearBuds and with AirPods. To evaluate against baseline methods, we use quantitative metrics on the test set of the synthetic data and hardware data described in section \ref{sec:datasets}. Finally, we conduct several ablation studies with the synthetic dataset to show how various factors influence our speech enhancement quality. The system latency on a variety of mobile devices is also reported.


\subsection{In-the-Wild User Study}\label{sec:mos} 
We conduct a user speaking and listening study to evaluate the quality of the output from our network in real situations. The procedure and results are described in the following sections.




% As described in section \ref{sec:nn}, in our hybrid network we apply an additional learned, low-cost spectrogram mask to clean unpleasant artifacts that surfaced when resource-constraining the Conv-TasNet architecture.
% As seen in Table \ref{table:results}, this change is not well characterized by SI-SDRi metric as the SI-SDRi of our CB-Conv-TasNet model did not differ from that of our hybridized, CB-Net architecture. So,  we conducted a subjective listening test to compare these two conditions.                
\subsubsection{Recording Procedure}
Various individuals wore a pair of ClearBuds and read excerpts from project Gutenberg while located in a noisy environment. These enviornments included a coffee shop, a noisy intersection, and an outdoor park. The environments featured ringing phones, cross-talk from other people, ambient music, a crying baby, opening/closing doors, driving vehicles, and street noise, amongst other common sounds. In total 10 different speakers were captured for a total of X hours of speech in Y environments.

\subsubsection{Evaluation Procedure} Twenty-five participants (8 female, 17 male, mean age 28) were recruited for an online listening survey. Each participant listened to 11 samples (each between 20--60 seconds). Each speech sample was processed and presented three ways: (1) the original input sample, (2) CB-Conv-TasNet, and (3) CB-Net, yielding a total of 25$\times$11$\times$3 $=$ 825 rating samples.

Participants were encouraged to use audio equipment they would typically use for a call. Eleven used earbuds, eight used laptop speakers, three used headphones, and two used phone speakers. The survey took about 25 minutes per participant. As is typical with noise suppression systems, participants were asked to give ratings in two categories: the intrusiveness of the noise and overall quality (mean opinion score - MOS):

\begin{small}
\begin{enumerate}
    \item \textbf{Noise suppression: }\textit{How INTRUSIVE/NOTICEABLE were the BACKGROUND sounds? 1 - Very intrusive, 2 - Somewhat intrusive, 3 - Noticeable, but not intrusive, 4 - Slightly noticeable, 5 - Not noticeable}
    \item \textbf{MOS: }\textit{If this were a phone call with another person, How was your OVERALL experience? 1 - Bad, 2 - Poor, 3 - Fair, 4 - Good, 5 - Excellent}  
\end{enumerate}
\end{small}

\subsubsection{Results}
Noise intrusiveness and MOS values for the original microphone, CB-Conv-TasNet, and CB-Net are provided in Figure \ref{fig:mos-study-results}.
As expected, applying CB-Conv-TasNet to the original audio helped suppress noise dramatically, increasing opinion score from 2.08 (slight better than \textit{2 - Somewhat intrusive}) to 3.29 (between \textit{3 - Noticeable, but not intrusive} and \textit{4 - Slightly noticeable}).
The light-touch, spectrogram-masking clean up method featured in CB-Net increased opinion score significantly (p<0.001) to  3.82, indicating the method did indeed further suppress perceptually annoying noise artifacts.
Importantly, this step also increased overall MOS. While users did not prefer (p>0.05) CB-Conv-TasNet (2.62) to the original input (2.54) due to artifacts introduced, they did significantly (p<0.001) prefer the CB-Net (3.06), an increase of 0.52 opinion score points from the input.
While this may not sound like a large difference, this magnitude increase is not unsubstantial. For example, in the recent, flagship ICASSP 2021 Deep Suppression Noise Challenge \cite{icaasp_dns}, which consists of state-of-the-art, real-time algorithms run on a quad-core desktop CPU, the winning submission increased MOS by 0.57 opinion score points \cite{icaasp_dns_results}.



% Further, to demonstrate our hybridized network's subjective background reduction and speech quality aspects, we run a  user study to compare the noise and speech performance amongst our mobile-deployed network architectures.

\subsection{Comparison against AirPods} \label{sec:endtoend}

To compare against commercially available wireless speech enhancement headphones, we numerically evaluate our end-to-end system against the Apple AirPods Pro headset connected to the same mobile device (iPhone 12 Pro). 

\subsubsection{Procedure} A foam mannequin head with a speaker (Sony SBS-XB12) inserted into its artificial mouth uttered one hundred VCTK samples from the test partition.
Ambient environmental sound (from WHAM! dataset) was played via four monitors (PreSonus Eris E3.5) positioned to fill 3 meter by 4 meter room, and background voice (also VCTK) was played from a monitor positioned 0.4 meters from head on the right.
The exact set up configuration can be found as a supplementary figure.

To create a repeatable soundscape for each test condition, all speakers were driven through a common USB interface (PreSonus 1810c) ensuring the same time-alignment and loudness between test conditions.
Since Apple AirPods Pro beamforming cannot be toggled on and off, we cannot calculate an SI-SDR increase, and therefore report output SI-SDR.
To establish a baseline against which to calculate SI-SDR ratio, we record a clean target voice through each headset.
Ambient noise SNR ranged between 0dB and 16dB with respect to target voice. Qualitatively, this sounded like a person speaking loudly in a noisy bar or cafe. Finally, background voice SNR ranged between 6dB and 12dB, qualitatively sounding like a person speaking from a meter or two away.

% %Loudness of target voice was about -22 dB as measured in recorded samples via ClearBud.

% During recording, qualitatively, it sounded like somebody talking loudly the room.
% %Loudness of ambient noise ranged between -38 and -22 dB.
% In input recorded samples, ambient noise SNR ranged between 0 dB and 16 dB with respect to target voice.
% Qualitatively, it sounded like a loud bar or a dense gathering.
%Loudness of side voice ranged -34 dB and -28 dB, 
% Side voice SNR ranged between 6 dB and 12 dB, qualitatively sounding like somebody speaking a meter or two away.

% \begin{table*}
%     %\vspace{-5mm}
% 	\centering
% 	\label{tab:real}
% 	\caption{Comparison against AirPods Pro. Numbers reported are the output SI-SDR (note: not SI-SDRi).}
% 	\small
% 	\begin{tabular}{c|ccc}
% 		\toprule
% 		& \multicolumn{3}{c}{Real Environment} \\  
% 		\midrule
% 		End-to-End System & {Target Voice + BG} & {Target Voice + BV} & {Target + BV + BG} \\
% 		\noalign{\vskip 1mm} 
% 		\hline
% 		\noalign{\vskip 1mm} 
% 		\textbf{ClearBuds}  & 15.40 & 19.09 & 15.21 \\
% 		Apple AirPods Pro & 10.17 & 10.48 & 8.27 \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{fig:airpods}
% 	\vspace{-0.15in}
% \end{table*}

\begin{figure}
\vskip -0.1in
\centering
\includegraphics[width=0.9\linewidth]{figures/AirPods_study_graph.png}
\caption{Comparison against AirPods Pro. Numbers reported are the output SI-SDR (note: not SI-SDRi). ClearBuds exceeds in three conditions: target voice plus background noise, target voice plus background voice, target voice plus background voice and noise. Target voice and background voice samples from VCTK representing a range of unseen speakers across gender and accent. Background noise from WHAM representing a range of indoor and outdoor environments. Data collected with mannequin head with artificial mouth sitting and array of background monitor speakers.}
\vskip -0.2in
\label{fig:airpods}
\end{figure}


\subsubsection{Results} We report output SDR from ClearBuds and Apple AirPods Pro in Figure ~\ref{fig:airpods}. To calculate output SDR, we align individual one second chunks and take the logarithmic mean across 250 chunks. We find that ClearBuds exhibits higher output SDR across all test conditions as compared to the beamforming utilized by the Apple AirPods Pro.

% Since Apple AirPods Pro do not zero pad dropped packets, misalignment can occur between test condition recording and reference recording over time, making it challenging to calculate SDR across all one hundred VCTK utterances at once. To overcome this, we align individual one second chunks and take the logarithmic mean across 250 chunks.


\subsection{Network Evaluation and Comparisons}

\begin{table*}[t]
    \label{tab:sdr-results}
    %\vspace{-5mm}
	\centering
	\caption{ Quantitative results on real and synthetic data. We show results for a target voice speaking in three noise scenarios: (1) Background noise (BG), (2) Background voice (BV), and (3) Background noise and background voice (BG and BV). Numbers reported are scale-invariant signal-to-distortion ratio increase (SI-SDRi). Ideal ratio mask (IRM) and ideal binary mask (IBM) are the oracle results for comparison that use the ground truth voice.}
	\small
	\begin{tabular}{c|ccc|ccc}
		\toprule
		& \multicolumn{3}{c}{SDR (std. dev.)} & \multicolumn{3}{c}{PESQ (std. dev.)} \\  
		\noalign{\vskip 0.3mm}    
% 		\toprule
		\midrule
		\noalign{\vskip 0.1mm}    
		Method & \shortstack{Target with\\ BG} & \shortstack{Target with\\ BV} & \shortstack{Target with\\ BV + BG} & \shortstack{Target with\\ BG} & \shortstack{Target with\\ BV} & \shortstack{Target with\\ BV + BG} \\
		\noalign{\vskip 1mm}    
		\hline
		\noalign{\vskip 1mm}    
		\textbf{CB-Net} & 11.58+-2.8 & 10.54 & 9.54 & 9.47 & 9.31 & 8.75 \\
		CB-Conv-TasNet   & 11.60 & 11.17 & 9.87 & 9.63 & 9.11 & 8.41 \\
		CB-Conv-TasNet Single Mic & 6.36 & 1.25 & 5.77 & 6.08 & 1.12 & 5.89 \\
 		CB-UNet & 2.55 & -0.36 & 1.51 & 1.60 & -0.16 & 1.30 \\
		Facebook Denoiser  & 6.75 & 1.55 & 5.98 & 5.89 & 1.169 & 5.62 \\
		Ideal Ratio Mask (IRM)  & 11.92 & 12.91 & 12.93 & 12.90 & 11.66 & 12.14 \\
		Ideal Binary Mask (IBM)  & 10.61 & 11.54 & 10.90 & 10.05 & 11.06  & 11.01 \\
		\bottomrule
	\end{tabular}
	\label{table:results}
\end{table*}


\subsubsection{Procedure} For numerical metrics and comparisons to other baseline methods, we use the popular metric \textit{scale-invariant signal-to-distortion ratio} (SI-SDR) \cite{sdr}. The SI-SDR of ground truth is computed relative to the noisy mixture and then to the network output. When reporting the increase from the input to output SI-SDR, we use the label SI-SDR improvement (SI-SDRi). Notice that we cannot compute metrics such as SI-SDR or PESQ on fully real recordings because a clean ground truth is required. Therefore we use our synthetic and hardware datasets where noisy mixtures are produced by mixing a clean ground truth and other interfering noises. \\

Results for numerical experiments are shown in Table \ref{table:results}. For a deep learning baseline in the waveform domain, we choose the causal Demucs model described in \cite{demucsreal}. This is a single channel method which was recently shown to outperform many other deep learning baselines and runs real-time on a laptop CPU. To compare with spectrogram based methods, we use the Oracle baselines based on the time-frequency representations. These baselines, ideal ratio mask (IRM) and ideal binary mask (IBM) \cite{sigsep, wang2005ideal}, use the ground truth voice to calculate the best possible result that can be obtained by masking a noisy spectrogram. As an ablation study, we report results with each individual component of the network, given by \textit{CB-Conv-TasNet} and \textit{CB-UNet}. We also show results when the multi-channel part of our network, \textit{CB-Conv-TasNet}, only has access to one microphone, labeled as \textit{CB-Conv-TasNet Single Mic}. This explicitly shows the advantage of using two microphones with our network. In the supplementary materials, we also show qualitative comparisons against Krisp \cite{krisp}, a commercial noise suppression system that shows strong performance. 

There are only a few deep learning methods that tackle binaural speech separation for mobile processing, and the most relevant ones, such as \cite{binaural_osu} and \cite{han2020realtime}, do not have publicly available code to test against.

\subsubsection{Results} As shown in Table \ref{table:results}, our binaural method is comparable to the best possible results that can be obtained by a spectrogram masking method. We also show an improvement over waveform based deep learning methods that only use a single microphone input. In particular, the improvement is greatest when there are two speakers present (Target Voice + Background Voice). This is because single channel methods can only rely on voice characteristics, whereas our network also uses spatial cues to separate the speaker of interest. Although \textit{CB-Net} shows similar performance to \textit{CB-Conv-TasNet}, subjective evaluation shows that \textit{CB-Net} is far superior to human listeners (see section~\ref{sec:mos}).

% \subsubsection{Results} Discuss results here

\subsection{Latency} Mouth-to-ear delay is defined as the time it takes from speech to exit the speaker's mouth and reach the listener's ear on the other end of the call. The International Telecommunication Union Telecommunication Standardization Sector (ITU-T) G.114 recommendation regarding mouth-to-ear delay indicates that most users are ``very satisfied'' as long as the latency does not exceed 200ms \cite{g.114}. In our end-to-end system, we targeted a one-way latency of 100ms prior to uplink, leaving up to 100ms of network delay to move an IP packet from source to destination.

With a 180-sample PCM buffer being filled at 31.250kHz, there is a 5.76ms delay prior to the samples reaching BLE stack. Once these samples reach the radio hardware, there is a worst-case additional latency of 7.5ms as defined by the minimum BLE connection interval supported by Bluetooth 5.0 \cite{bt5}. However, at the time of writing, the latest iOS supports a minimum BLE connection interval of 15ms. After the samples reach the mobile phone, we wait for 67.2ms to receive enough samples to run a forward pass of our network. From the latency table, we see that our network has a run-time of 21.4ms on an iPhone 12 Pro. Added together, we have a  latency of 109ms, leaving 91ms for network delay.

\subsection{Additional network evaluations} We evaluate various aspects of the design including its performance with angle of background voice, multi-path and reverberant environments as well as separation between microphones. 


\paragraph{Angle of Background Voice} \label{sec:angular}

\begin{figure*}
\centering     %%% not \center
\subfigure[]{\label{fig:angle}\includegraphics[width=0.32\textwidth]{figures/angle-graph.png}}\hfill
\subfigure[]{\label{fig:reverb}\includegraphics[width=0.32\textwidth]{figures/reverb-graph.png}}\hfill
\subfigure[]{\label{fig:head-width}\includegraphics[width=0.32\textwidth]{figures/ear-distance-graph.png}}
\vskip -0.15in
\caption{(a) Performance against angle of background voice. When the background voice is close to the front-back plane ($0^\circ$), there are no spatial cues and the separation ability worsens. Our performance improves when the angle extends past 12 degrees. (b) Performance against amount of reverberation in an indoor room. RT60 (in seconds) measures how long sound takes to decay by 60 dB in a space with a diffuse soundfield. (c) Performance as distance between ears increases. No noticeable impact to performance across varying head widths.}
\label{fig:ml-performance}
\vskip -0.2in
\end{figure*}

The ability of our network to separate the target voice from a background voice is based on utilizing the time difference of arrival to the binaural microphones. Because we only have two microphones, this ability is limited when the background voice is in the front-back plane of the speaker. In this case, the background voice will arrive at each microphone simultaneously, and there will be no spatial cues to separate the two voices.  To illustrate this effect, we graph the separation performance as a function of the angle of the background voice in Figure \ref{fig:angle}. 

\paragraph{Multi-path and  Reverberant Environments}

We show that our method works in a variety of reverberant conditions, including those more reverberant than seen during training. Synthetically generated mixtures are generated using the pyroomacoustics library as described in section \ref{sec:synthetic-data}, with the RT60 value randomly chosen between 0 and 4s. We generate 200 examples and plot the SI-SDRi compared to the RT60 in Figure~\ref{fig:reverb}. Our method shows only a slight decrease in performance as the reverberation of the environment increases. Because the target speaker is physically close to the microphone array, our setup is generally less affected by reverberations than other kinds of source separation problems where the target speaker may be further away.

\paragraph{Separation Between Microphones} We also show that our method generalizes to different head sizes where the distance between the microphones may be different. We generate 200 synthetic samples using the same method described in Section \ref{sec:synthetic-data}, where the distance between the microphones is randomly chosen between 10 and 25cm. Because the target speaker is in the middle of the microphone array, the target signal will arrive at both mics simultaneously regardless of the microphone distance. The results in  Figure~\ref{fig:head-width} show little change in performance even with microphone distances greatly different than used during training.


\begin{table}%[b]
	\centering
	\caption{ Network runtime measured on previous 3 generations of iPhone. Our network operates in chunk sizes of 22.4ms. As long as the network runtime is less than this duration, it can operate in real-time.}
	\label{tab:latency}
	\small
	\begin{tabular}{ccccc}
		\toprule
		Device & Full Conv-TasNet & CB-Conv-TasNet & \textbf{CB-Net} \\
		\noalign{\vskip 0.5mm} 
		\hline
		\noalign{\vskip 1mm} 
		iPhone 12 Pro & 155.5ms & 17.5ms & 21.4ms \\
		iPhone 11 & 165.4ms & 18.6ms & 22.7ms \\
		iPhone XS & 241.5ms & 27.2ms &  33.0ms \\
		\hline
		\noalign{\vskip 1mm} 
		FLOPs & 1078M & 97M & 131M \\
% 		iPhone 12 Pro & 155.5ms & 17.5ms & 3.9ms & 21.4ms \\
% 		iPhone 11 & 165.4ms & 18.6ms & 4.1ms & 22.7ms \\
% 		iPhone XS & 241.5 & 27.2ms & 5.8ms &  33.0ms \\
		\bottomrule
	\end{tabular}

	%\vspace{-8mm}
	\vskip -0.15in
\end{table}




==> sections/6-broader_impact.tex <==
\section{Broader Impact}
\begin{help-env}
This research aims to bridge together the state-of-the-art learnings from blind audio source separation and in-ear mobile systems. The impacts of this research would benefit anyone taking calls in loud or noisy environments.

 By open-sourcing the hardware platform and collected datasets, this work will also kickstart future research among mobile system and machine learning researchers to design novel algorithms around binaural audio data.
 \cite{defossez2019music}
 [EXPAND]
 
 \end{help-env}

==> sections/9-checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{Will include in supplementary.}
  \item Did you include the license to the code and datasets? \answerYes{Will include in supplementary.}
  \item Did you include the license to the code and datasets? \answerYes{Will include in supplementary.}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Will include in supplementary.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{This will be provided in the supplementary.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/999-sections_from_template.tex <==
\section{Submission of papers to NeurIPS 2021}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2021 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.

The margins in 2021 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2021.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2021 is \verb+neurips_2021.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2021.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2021+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2021}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2021/PaperInformation/FundingDisclosure}.

Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip

{
\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix

\section{Appendix}

Optionally include extra information (complete proofs, additional experiments and plots) in the appendix.
This section will often be part of the supplemental material.


